A multiwavelength survey of HI-excess galaxies with surprisingly inefficient star formation

We present the results of a multiwavelength survey of HI-excess galaxies, an intriguing population with large HI reservoirs associated with little current star formation. These galaxies have stellar masses $M_{\star} >10^{10}$ M$_{\odot}$, and were identified as outliers in the gas fraction vs. NUV$-r$ color and stellar mass surface density scaling relations based on the GALEX Arecibo SDSS Survey (GASS). We obtained HI interferometry with the GMRT, Keck optical long-slit spectroscopy and deep optical imaging (where available) for four galaxies. Our analysis reveals multiple possible reasons for the HI excess in these systems. One galaxy, AGC 10111, shows an HI disk that is counter-rotating with respect to the stellar bulge, a clear indication of external origin of the gas. Another galaxy appears to host a Malin 1-type disk, where a large specific angular momentum has to be invoked to explain the extreme $M_{\rm HI}$/$M_{\star}$ ratio of 166$\%$. The other two galaxies have early-type morphology with very high gas fractions. The lack of merger signatures (unsettled gas, stellar shells and streams) in these systems suggests that these gas-rich disks have been built several Gyr-s ago, but it remains unclear how the gas reservoirs were assembled. Numerical simulations of large cosmological volumes are needed to gain insight into the formation of these rare and interesting systems.

==> Tex_files/All.tex <==

\section{Appendix}\label{Sec:Appendix}


\begin{figure*}
\includegraphics[width=.218\textwidth]{Plots/Spectra_G20339.png}
\includegraphics[width=.22\textwidth]{Plots/Spectra_J1126.png}
\includegraphics[width=.222\textwidth]{Plots/Spectra_J1558.png}
\includegraphics[width=.206\textwidth]{Plots/Spectra_J1605.png}
\begin{center}\caption{Comparison between the Arecibo (black line) vs. GMRT (red line) \HI\ spectra. 
{\bf The single-dish spectrum of AGC 192040 is from GASS, the other three galaxies are extracted from ALFALFA.}
The galaxies are AGC 192040 (left), AGC 731712 (second to the left), AGC 10111 (second to the right), AGC 263047 (right).}\label{fig:Spectra}
\end{center}
\end{figure*}



\begin{table*}
  \caption{Properties of galaxies in the environment of the \HI-excess sample. Col.1 Target AGC galaxy; Col.2 SDSS identification number; Col.3 redshift; Col.4; line-of-sight velocity difference relative to the target galaxy; Col.5 projected distance from the \HI-excess galaxy; Col.6 stellar mass; Col.7 \HI\ mass; Col.8 Membership to the target galaxy (named in brackets), where $1$ marks gravitationally bounded cases and $0$ marks non-members (see text). }\label{table:appendix}
 
   \begin{center}
    \begin{threeparttable}
     \begin{tabular}{l l l l l l l c} 		
   % &  & References\\ 	
\hline									     
Target AGC galaxy & SDSS ID  & z   & $v_{\rm los}$ & $d_{\rm proj}$       & log($M_{\star}$) & log($M_{\rm \HI}$) & Membership\\   
              &           &             &    km s$^{-1}$  &  kpc    &[\msun]           &  [\msun]           & \\
\hline	
%(G20339bigger)
AGC 192040 & SDSSJ094645.18+105414.0 & 0.047153            & 99$^{\dagger}$ & 818 &  10.13 & $<$9.4 & 0 \\ 
%(G20339)
           & SDSSJ094706.15+104957.0 & 0.047404            & 24$^{\dagger}$ & 451 &  9.58  & $<$9.6 & 1 \\
%(J1126-dwarf) 
AGC 731712 & SDSSJ112633.66+240100.3 & 0.026450 $^{\star}$ & 202            & 42  &  8.76  & 8.21   & 0  \\
%(J1126)
           & SDSSJ112650.36+240613.2 & 0.019661 $^{\star}$ & 1832           & 167 &  9.07  & 8.87   & 0  \\
%(J1558)
AGC 10111 & SDSSJ155836.37+130503.9 & 0.034413             & 55             & 314 &  10.01 & 9.69   & 1 

\end{tabular}
    \begin{tablenotes}
   %  {\bf References.} (1) Catinella et al. (2010); (2) Saintonge et al. (2011a)
     \item[$\star$]  based on \HI\ velocity.
     \item[$\dagger$]  based on SDSS redshift.
    	\end{tablenotes}
    	   \end{threeparttable}
\end{center}
\end{table*}


\begin{figure*}
\includegraphics[width=.75\textwidth]{Plots/G20339_env.png}
\begin{center}\caption{The environment of AGC 192040 (marked in blue contours). The surrounding galaxies with \HI\ non-detections are marked as red boxes.}\label{fig:G20339_env}
\end{center}
\end{figure*}


\begin{figure*}
\includegraphics[width=.75\textwidth]{Plots/J1126_env.png}
\begin{center}\caption{The environment of AGC 731712. The central galaxy is marked in blue as in Fig. \ref{fig:G20339_env}, and the \HI\ contours associated with dwarf galaxies in the surrounding volume are shown in red.}\label{fig:J1126_env}
\end{center}
\end{figure*}


\begin{figure*}
\includegraphics[width=.75\textwidth]{Plots/J1558_env.png}
\begin{center}\caption{AGC 10111 is marked in blue. The other \HI\ detection in the environment of this galaxy is marked in red. }\label{fig:J1558_env}
\end{center}
\end{figure*}


%\topmargin2cm
%\textheight29cm
%\newpage
%\pagestyle{empty}
%\begin{figure*}
%\begin{picture}(600,600)(0,0)
%\graphpaper(-50,-100)(500,700)
%\put(-60,390){\framebox(290,140){}}
%\put(-20,475){\includegraphics[width=.22\textwidth]{Plots/SDSS_G20339.png}}
%\put(90,460){\includegraphics[width=.9\textwidth]{Plots/Collection_G20339.png}}
%\put(-20,320){\includegraphics[width=.22\textwidth]{Plots/SDSS_J1126.png}}
%\put(90,310){\includegraphics[width=.9\textwidth]{Plots/Collection_J1126.png}}
%\put(-20,175){\includegraphics[width=.22\textwidth]{Plots/SDSS_J1558.png}}
%\put(90,160){\includegraphics[width=.9\textwidth]{Plots/Collection_J1558.png}}
%\put(-20,20){\includegraphics[width=.22\textwidth]{Plots/SDSS_J1605.png}}
%\put(90,10){\includegraphics[width=.9\textwidth]{Plots/Collection_J1605.png}}
%\end{picture}
%\caption{Bla}
%\end{figure*}



\begin{figure*}
\includegraphics[width=.95\textwidth]{Plots/DeepOpt.png}
\begin{center}\caption{Deep optical images of AGC 192040 (VLT, left), AGC 731712 (CFHT, middle), and AGC 263047 (CFHT, right). }\label{fig:Collection_Optical}
\end{center}
\end{figure*}



\begin{figure*}
\includegraphics[width=.43\textwidth]{Plots/PV_G20339.png}
\includegraphics[width=.43\textwidth]{Plots/PV_J1126.png}
\includegraphics[width=.45\textwidth]{Plots/PV_J1558.png}
\includegraphics[width=.44\textwidth]{Plots/PV_J1605.png}
\begin{center}\caption{\HI\ position-velocity diagrams extracted along the position angles of the Keck observations. The \HI\ is marked with dark colours. Measurements based on the H$\beta$ (4861.3$\AA$), H$\gamma$ (4340.5$\AA$), and OIII (4958.9$\AA$, 5006.8$\AA$) emission lines are shown as cyan points. The NaI (5892.5$\AA$) and E-band (5269.0$\AA$) absorption line measurements are marked in red. The red ellipse marks the location of the \HI\ tail in AGC 192040, although we remark that this gas of cloud has a more prominent detection along a different position angle (not shown). In the diagram of AGC 731712 the dark blue point marks the Keck detection of a dwarf galaxy. } \label{fig:HI_pv}
%The galaxies are: AGC 192040 (upper left), AGC 731712 (upper right), AGC 10111 (lower left), AGC 263047 (lower right). 
\end{center}
\end{figure*}


\section{Observations and data reduction}\label{Sec:DataReduction}

% 10 hours is lost due to the observed frequency setting not being fine-tuned.
%The data were cleaned of RFI, and the continuum was subtracted by fitting a low order polynomial to the line-free channels.  

\subsection{Deep Optical Imaging}

%- See first column of Fig. \ref{fig:Collection}. Data collected from VLT and CFHT. Data reduction.
%as part of program 088.B-0253(A) (PI, Catinella)

We obtained deep optical images for three of the galaxies in this sample. Very Large Telsecope - FOcal Reducer/low dispersion Spectrograph 2 (VLT/FORS2) observations of AGC 192040 were undertaken in 2011-2012, and include 15x240s exposures in the R filter. These observations were reduced with the standard ESO pipeline in the Reflex environment \citep{Freudling2013}. Archival images for AGC 731712 and AGC 263047 were obtained from the CFHT archive\footnote{$http://www.cadc-ccda.hia-iha.nrc-cnrc.gc.ca/en/search/$}. AGC 731712 was observed in B and V filters for 840s and 480s respectively, by the CFH12K Mosaic camera in 2001; AGC 263047 was observed in the r filter for 3x240s with the MegaPrime camera in 2008. Standard Level 2 calibrated data were obtained through the CADC. An additional dark sky flat field correction was applied to observations of all three galaxies and photometric calibrations were made with foreground stars measured by SDSS DR9 \citep{Ahn2012}, following the methodology of \cite{Janowiecki2015}. 
{\bf The resulting three images are shown in Fig. \ref{fig:Collection_Optical}. We note that no deep images are available for AGC 10111.} 



\subsection{Interferometric HI observations}

GMRT \HI\ observations were carried out between Aug 2015 - Dec 2016. Each galaxy was observed for 25 hours, except for AGC 263047 where only 7 hours of observations are available. The 16 MHz bandwidth was covered by 512 frequency channels corresponding to a velocity resolution of $\sim$15 km s$^{-1}$ after Hanning smoothing. The data were calibrated and reduced following standard procedures in the Common Astronomy Software Applications (CASA, \citealt{McMullin2007}) package. The \HI\ cubes were created with task $\it clean$ using natural weighting to maximise the signal-to-noise ratio. GMRT has a $\sim4$ arcsec spatial resolution at 1.4 GHz. The data were tapered to lower resolution, a common $\sim15$ arcsec beam size, in order to improve the \HI\ brightness sensitivity. The $smallscale$ bias parameter was set to zero to avoid scaling of the \HI\ flux. After Hanning smoothing, the 3$\sigma$ rms noise is 0.3 mJy beam$^{-1}$ channel$^{-1}$ in AGC 263047, and 0.2 mJy beam$^{-1}$ channel$^{-1}$ in the other three \HI\ cubes. {\bf The resulting GMRT spectra are shown in Fig. \ref{fig:Spectra} along with the GASS and ALFALFA spectra of the galaxies for comparison. The GMRT observations successfully recover the flux of the single dish measurements.} The integrated intensity (zeroth-moment) and velocity field (first-moment) maps presented in Fig. \ref{fig:Collection} were created from the data cubes using task {\it immoments}. The zeroth-moment map was converted into column density following \cite{Morganti2007}.
%The GMRT \HI\ spectra are compared to the ALFALFA measurements in Fig. \ref{fig:Spectra}, showing that the ALFALFA \HI\ mass is successfully recovered within the sample. 

%In AGC 192040 the GMRT \HI\ mass is 20$\%$ smaller than in ALFALFA, suggesting that part of the gas is too diffuse to be detected at the 4$\times$10$^{19}$ cm$^{-2}$ column density limit of the GMRT observations. This is also supported by the unsettled nature of the gas in Fig. \ref{fig:Collection}. In the other three galaxies 


\subsection{Optical spectroscopy}

The four galaxies were observed with the Echelette Spectrograph and Imager (ESI) on the 10m Keck II telescope at Mauna Kea on 29 Mar 2016. We used ESI in low-dispersion mode with a slit 1" wide and 8' long, aligned with the major axis of each galaxy. The average spectral resolution was R$\sim$3000 across our range from $\sim$4000A to $\sim$8000A. The spatial resolution along the slit direction is $\sim$1". We integrated for 6x1200s on each target. % and also obtained 2x900s integrations with an alternate position angle on AGC 731712 to measure the redshift of its nearby dwarf galaxy (see Section \ref{sec:multiwavelength}).

These longslit spectra were reduced with the standard processing tools in IRAF\footnote{IRAF is distributed by the National Optical Astronomy Observatory, which is operated by the Association of Universities for Research in Astronomy (AURA) under a cooperative agreement with the National Science Foundation.}, and the observations were corrected for overscan, bias, flat field, cosmic rays, and rotation. Multiple exposures of each target were averaged together and re-projected to a common wavelength scale using observations of calibration lamp spectra. 

For each target, we fit Gaussian profiles to the nebular emission and stellar absorption lines at each position along the slit and determine the barycentric velocity of each feature. All four galaxies in this sample show emission lines beyond their bright central regions, supporting the presence of star-forming regions as suggested by the UV images (see Fig. \ref{fig:Collection}).  
{\bf The ionized gas and stellar kinematics are compared to the \HI\ kinematics in Fig. \ref{fig:HI_pv}. 
The \HI\ pv-diagrams were extracted along the position angle and central position of the Keck slit observations to perform this comparison.}

%In all cases, the ionized and neutral gas kinematics are consistent in the outskirts of the galaxies, but sometimes the central stellar kinematics seem to deviate from that rotation (see AGC 10111). 


\subsection{UV imaging}

We use GALEX FUV images for studying the SFR across our sample. The maps of the four \HI-excess galaxies are retrieved from the GALEX All Sky Survey (AIS) through the Multimission Archive at Space Telescope Science Institute (MAST). The AIS has observed over 26,000 square degrees of sky with 100s exposure time, reaching a depth of m$_{AB}$ = 20.5. The FUV maps are background subtracted in IRAF, the photon counts are converted into flux, then into SFR{\bf, following \cite{Bigiel2010}}. We smooth the maps to 15" to match the resolution of the \HI\ data. The pixel size is set to be 3" in both the \HI\ and FUV maps, corresponding to 1.5-2.7 kpc in the redshift range of the observations. The resulting maps are shown in Fig. \ref{fig:Collection} (second to the left). %, the distribution of FUV regions coincide with the highest column density regions of the \HI\ disks.



\section{Discussion}\label{Sec:Discussion}

In this section we focus on discussing the $>2.5\sigma$ \HI\ excess in relation to the star-forming and structural properties in our sample.


The $\mu_{\star}$ vs. gas fraction relation in Fig. \ref{fig:diagnostics} (right panel) reveals that the \HI-excess sample has high gas fractions for galaxies of the same structure. Our sample mainly consists of bulge-dominated galaxies (see optical images in Fig. \ref{fig:Collection_Optical}), thus we use the \atlas\ representative sample of early-type galaxies to put the gas-richness of our \HI-excess galaxies into context. 
% to understand how gas-rich \HI-excess galaxies truly are compared to galaxies of a similar kind. 
\atlas\ has surveyed the \HI\ content of 166 early-type galaxies in- and outside of the Virgo cluster, and detected $10^8 - 10^{10}$ \msun\ of \HI\ in about half of the sample \citep{Serra2012}. The largest gas fraction among the settled disks of \atlas\ galaxies is log($M_{\rm HI}$/$M_{\star}$)$ = -0.8$, whereas the gas fraction of the four galaxies studied in this paper varies between $-0.093 \leq$ log($M_{\rm HI}$/$M_{\star}$) $\leq 0.222$. Thus, \HI-excess galaxies are on average 10 times more \HI-rich compared to the \atlas\ sample.
This explains the outstanding position of the galaxies in Fig. \ref{fig:diagnostics} (right panel), showing that \HI-excess galaxies are the most gas-rich amongst bulge-dominated systems. So how can these galaxies keep such large gas reservoirs?


%********************
\HI-excess galaxies are distributed at the upper envelope of the NUV$-r$ vs. gas fraction relation in Fig. \ref{fig:diagnostics} (left panel), revealing a clear disconnection between \HI\ and star-forming properties. We explore whether this is due to the galaxies having too much gas, or due to inefficient star formation in the low surface brightness disks.
In Fig. \ref{fig:logGF_Mstar}, AGC 192040 is the only galaxy among the studied sample with expectionally high gas fraction for its stellar mass. In fact, the log$M_{\rm HI}$(\msun) = 10.76 \HI\ mass of this galaxy is almost two times higher than its stellar mass. 
Neither HIghMass, nor the sample by \cite{Lemonias2014} contains log$M_{\star}$(\msun) $\sim 10.5$ stellar mass galaxies with such high gas fractions, however a few similarly gas-rich systems were found in the HIX sample by \cite{Lutz2017}. Looking at Fig. \ref{fig:logGF_Mstar}, the other three \HI-excess galaxies have normal gas fractions for their stellar mass, suggesting that these are not particularly gas rich for their stellar content. This leaves us with the conclusion that low star-forming efficiency pushes \HI-excess galaxies to the upper envelope of the NUV$-r$ vs. gas fraction relation.


Low star-forming efficiency is also supported by the KS relation in Fig. \ref{fig:KS}, where we show that the \HI-based gas depletion timescales at the current rate of star formation are of the order of 10$^{10} - 10^{11}$ years. This is 10 - 100 times longer than the SFR efficiency in "normal" SF galaxies \citep{Schiminovich2010, Gereb2015}. The low molecular gas fraction detected in AGC 192040 suggests that CO formation is a very inefficient process in the extended disk of this galaxy. Similar results were found for the \HI-excess galaxy GASS 3505, where CO observations by the COLD GASS survey yielded a log$M_{\rm H2}$(\msun) $<8.93$ upper limit, corresponding to a log($M_{\rm H2}/M_{\rm HI}$) $<-0.97$ molecular gas fraction. Molecular gas observations are not available for other galaxies in our sample. However, based on the available data we speculate that something is preventing the collapse of gas into molecular clumps in \HI-excess galaxies.


Given that \HI-excess galaxies are strong outliers in the stellar surface density vs. gas fraction relation in Fig. \ref{fig:diagnostics}, we also investigate whether galaxy structure can play a role in suppressing star formation.
Cosmological zoom-in simulations of merging spiral galaxies by \cite{Martig2009} suggest that the transition from a stellar disk to a spheroid is sufficient to prevent gravitational fragmentation of the gas due to the potential well being steeper and the disk self-gravity being reduced in the resulting spheroid.
This, so-called morphological quenching, scenario suggests that galaxies can turn 'red and dead' in the presence of a bulge without the removal of gas. 
Previously, \cite{Fabello2011} carried out an \HI\ stacking study of ALFALFA galaxies and found that on the red sequence, galaxies with higher concentration indices (a proxy for bulginess) have higher average gas fractions compared to galaxies with a low concentration index. Thus, their results are inconsistent with the morphological quenching scenario. 
We carry out a similar test by comparing \HI-excess galaxies to the spiral-dominated HIghMass sample. We expect \HI-excess galaxies to be more gas rich than late-type galaxies of the same colour if the morphological quenching scenario is true. The NUV$-r$ vs. gas fraction distribution of the two samples is presented in Fig. \ref{fig:diagnostics} (left),{\bf where HIghMass galaxies are marked as cyan squares. For this comparison the galaxies were selected to have log$M_{\star}$(M$_{\odot}$)$>10$ to match the GASS selection criteria. 
The extreme outlier from HIghMass is UGC 09234, a galaxy that fulfills our \HI-excess selection as already discussed in \cite{Gereb2016}.
Here we are only focusing on the four \HI-excess targets marked as coloured circles in Fig. \ref{fig:diagnostics}.  
These points do follow the HIghMass distribution when the star-forming outskirts are included in the colour measurements.
Given that the four \HI-excess galaxies with remeasured colours have similar gas fractions as HIghMass galaxies,
the morphological quenching scenario can not explain the low star-forming efficiency in our bulge-dominated \HI-excess sample.}

%The interpretation of the offset for the rest of the sample is warranted, as these measurements only take into account the colours of the central parts of \HI-excess galaxies.

{\bf In \cite{Gereb2016} we explored the multiwavelength properties of our prototype \HI-excess galaxy, GASS 3505, and found that its low star-forming efficiency can be attributed to low gas column densities in an extended \HI\ ring ($\sim$50 kpc radius). Using numerical simulations we showed that a GASS 3505-type galaxy can be created in a merger between a gas-rich and a bulge-dominated system. Our results also suggest that multiple events are needed to explain the large \HI\ mass ($10^{9.9}$ \msun) measured in this galaxy}.
Here, in Sec. \ref{sec:multiwavelength} we looked for signatures of external gas accretion in the current sample and found evidence for counter-rotation in AGC 10111. 
{\bf In fact, in our multiwavelength dataset this is the most clear evidence for gas accretion, emphasising that the combination of optical and \HI\ kinematic information will be crucial for the success of future gas accretion studies.} The $\sim50$ deg offset between the kinematic axis of these two gas phases points to a polar orientation of the \HI\ compared to the central bulge. 
Theoretical simulations \citep{Bekki1998, Spavone2010, bassett17c} successfully reproduce the formation of polar rings through external gas accretion either from the interagalactic medium or via gas-rich mergers.  \cite{Mapelli2015} finds that minor mergers between S${\rm 0}$ galaxies and their satellites can create long-lived polar rings with star formation that lasts $\sim$10 Gyr. This is similar to the timescales estimated for our sample. However, the $>10^{10}$ \msun\ of \HI\ masses detected in our sample are too large to originate from a single minor merger event, similarly to what found in GASS 3505.  

AGC 192040 is another galaxy where we find indications for a recent interaction in form of a kinematically decoupled gas tail. Stellar and UV components are both detected coinciding with the unsettled gas, making this tail a good candidate for being a minor merger remnant. 
However, AGC 192040 is an \HI-excess galaxy even without the 15$\%$ contribution of the tail to the total \HI\ mass, thus additional processes need to be invoked to explain the \HI-excess disk.
{\bf In fact, AGC 192040 has the most prominent disk among the sample in terms of its large log($M_{\rm HI}$/$M_{\star}$) $= 0.222$ gas fraction, and 65 kpc \HI\ radius (70" at z=0.047). This galaxy is comparable to a Malin 1-type low-surface brightness galaxy in terms of its gas richness \citep{Pickering1997, Lelli2010, Boissier2016}. AGC 192040 is less extreme than Malin 1 (which has a disk size of 130 kpc radius and \HI\ content of log$M_{\rm HI}$($M_{\odot}$) = 10.82), but it could be a similar type of object at slightly lower redshift (Malin 1 is at z=0.08). 
Theoretical work shows that an elevated specific angular momentum is able to keep the gas in extended, low surface density configuration like in Malin 1, where the gas becomes stable against gravitational fragmentation and consequent star formation \citep{Mo1998, Boissier2000, Kravtsov2013}. It has been suggested that high angular momentum is responsible for the accumulation of large \HI\ reservoirs in galaxies that are selected to be \HI-rich for their stellar content \citep{Huang2014, Lemonias2014, Lutz2017}. AGC 192040 satisfies the selection criteria of these \HI-rich samples based on Fig. \ref{fig:logGF_Mstar}, strengthening the assumption that high angular momentum is responsible for keeping the gas in an extended, \HI-rich configuration in AGC 192040. }

%However, most of the \HI-excess galaxies are not outliers in the $M_{\star}$ vs. gas fraction relation, reflecting their different selection.
  
In the remaining two galaxies (AGC 731712 and AGC 263047) the settled nature of the gas suggests that the \HI\ disks have been in place for at least one orbital time. This timescale is a few Gyr for massive galaxies ($>10^{10}$ M$_{\odot}$) with extended disks (tens of kpc-s) like the ones observed in our \HI-excess sample.
Despite the wealth of multi-wavelength data, it is still unclear how these galaxies gained and preserved their gas. {\bf AGC 731712 and AGC 263047 seem to be \atlas-type galaxies in terms of their large bulge-to-total ratios and extended \HI\ disks, however with larger \HI\ masses and gas fractions.
Numerical simulations are able to reproduce bulge-dominated galaxies with extended, gas-rich disks via major mergers between two gas-rich galaxies \citep{Naab2001, Barnes2002, Springel2005, Robertson2006}. This formation mechanism has been suggested to be responsible for the formation of \HI-systems like the ones observed in \atlas\ and other early-type galaxies \citep{Serra2006, Oosterloo2010, Serra2012}.}


In summary, the four galaxies studied in this paper seem to be a mixed bag, some of them {\bf show signatures of recent interactions} (AGC 192040), but it appears that the bulk of the \HI\ disks have been built at least a couple of Gyr ago. The diffuse nature of the extended outskirts, combined with low star-forming efficiencies points to a gradual build-up of the low surface brightness disks over an extended period of time like in a Malin 1-type galaxy \citep{Boissier2016}.{\bf \HI-excess galaxies are 1-2 orders of magnitude less efficient at converting their gas into stars than normal star-forming galaxies. However, \HI-excess galaxies are definitely not red and dead. There is usually a quick transition assumed to take place in galaxies as they move from the blue cloud to the red sequence in the color magnitude diagram \citep{Bell2004, Wyder2007, Schawinski2014}. Our sample reveals examples of galaxies at this intermediate stage. Based on the large gas masses and low star-forming efficiencies involved, the galaxies will remain in this state for a long time (more than 10 Gyr) as opposed to being transitional objects.



Thus, it appears that the gas fraction plane yields very unique and interesting objects. 
In order to understand the formation and evolution of these galaxies, hydrodynamic simulations of large volumes are needed in a cosmological context, where the accretion processes in galaxies and merger histories can be tracked. Both the Evolution and Assembly of GaLaxies and their Environments (EAGLE \citealt{Schaye2015}) and Illustris \citep{Nelson2015} simulations cover a volume of roughly (100 Mpc)$^3$. The volume density of \HI-excess galaxies is of the order of 10$^{-5}$ Mpc$^{-3}$ based on the sky regions convered by ALFALFA and GASS (in the redshift range $0.01 < z < 0.05$), thus the simulated volumes are clearly not enough to yield a statistically representative sample. 
Observationally, metallicity measurements can provide additional information on the build-up of the extended outksirts. Metal enrichment and the age of the stellar populations are strongly related through star-formation, thus metallicity measurements can help to constrain the formation timescales involved in the build-up of \HI-excess galaxies \citep{Moran2010}.
}


%In some of the galaxies large angular momentum seems to play a role in keeping the gas at the outskirts of galaxies (AGC 192040). We also see signatures of gas accretion in AGC 10111, suggesting that the low star-forming efficiency in this case is due to externally accreted gas. In the remaining two galaxies the picture is less clear, and these could be just scaled-up versions of \atlas-type galaxies in terms of their gas content.


%XXX - look up what metallicty plots exist! - what can we learn, refer to Luca
%Modeling to constrain the angular momentum -  there are no consistent samples to compare. 
 %Furthermore, simulations need to be able to reproduce the low surface brightness Universe (both gas and stars) to be able to compare with observations. XXX-what simluations?? - references
 %Furthermore, is smoothed particle simulations like  
 %CDM cosmological simulations of galaxy formation tend to produce dense and compact disks, as much angular momentum is lost during the hierarchical assemblage 
%\bibitem[\protect\citeauthoryear{Kaufmann et al.}{2007}]{Kaufman2007} Kaufmann T., Mayer L., Wadsley J., Stadel J., Moore B., 2007, MNRAS, 375, 53 


\begin{figure}
\includegraphics[width=.43\textwidth]{Plots/logGF_Mstar.png}
\begin{center}\caption{Gas fraction ($M_{\rm HI}/M_{\star}$) vs. stellar mass ($M_{\star}$) relation of \HI-excess galaxies (red points and coloured stars), and the underlying GASS sample (blue shaded regions). } \label{fig:logGF_Mstar}
%The galaxies are: AGC 192040 (upper left), AGC 731712 (upper right), AGC 10111 (lower left), AGC 263047 (lower right). 
\end{center}
\end{figure}


%Recent hydrodynamical simulations show that certain type of minor mergers also provide favorable conditions to form galaxies with extended gas configurations \citep{bassett17c}. The gas is more efficiently stripped by central galaxies with large bulge-to-total ratios in these simulations, due to higher stripping efficiency due to the shape and depth of the gravitational potential produced by the compact mass profile of the bulge.
%The simulations carried out for GASS 3505 supports this scenario, however one such event is unable to explain the large $>10^{10}$ M$_{\odot}$ gas masses detected in \HI-excess galaxies.


%In the previous sections we show that even after we include the outskirts, What is driving the 
%In this section we discuss possible scenarios that can explain the build-up of large-scale, stable disks like the ones observed in the \HI-excess sample, focusing on gas accretion processes. 
 
%What do we need from observations and simulations to understand these obejcts? 
%- metallicity
%- simulations: based on $\Lambda$CDM cosmology mainly produce compact disks, and they have a hard time producing extended, diffuse disks. Rob's simulations show that you can make extended rings in minor mergers, bu we need these simulations in a cosmological context.

%disk formation plays a role in 
%These galaxies are rare to find, but our study reveals a few ways to identify them:they either represent the high-end tail of the angular momentum distribution, they can be identified by kinematic misalignment between the HI and ionised phases of the gas, . but not all galaxies are the same. 
 %we would need to catch these galaxies at an earlier stage of their evolution.
%galaxy evolution studies in terms of the colour-magnitude diagram.
%There is usually a fast transition assumed between blue, star-forming and red inactive galaxies. \\
%
%- LSB galaxies contribute 50$\%$ of the light emitted by nearby galaxies. Due to the low SBs these often remain hidden in shallow surveys, but we can expect to find more in the future. \\
% \\
%- it also appears that gas accretion processes via mergers might play a role in rejuvenating some of these galaxies, like AGC 10111. \\


%\begin{figure*}
%\includegraphics[width=.43\textwidth]{Plots/Color_vs_GF.png}
%\includegraphics[width=.43\textwidth]{Plots/ATLAS3D_MH2_MHI.png}
%\begin{center}\caption{ } \label{fig:MorphQuench}
%The galaxies are: AGC 192040 (upper left), AGC 731712 (upper right), AGC 10111 (lower left), AGC 263047 (lower right). 
%\end{center}
%\end{figure*}


%Based on our results gas accretion processes are likely to play a role in rejuvenating otherwise passively evolving, bulge-dominated galaxies and thus introducing a scatter in the gas fraction scaling relations \citep{Cortese2009}.
%This will be addressed in a future work.
% detected in the tail is not enough to make this galaxy \HI-excess in the gas fraction plane, and it that the bulk of the gas has been sitting there for a while.
 % The \HI\ tail constitutes 15$\%$ of the total \HI\ mass, which is a reasonable amount to originate from a minor merger. 
%Thus, we can not rule out the possibility of smooth gas accretion as a source of gas in AGC 10111, and it is even more likely that multiple accretion events%, but this gas coud contribute to make this galaxy an outlier in the 

%Given the very few observational evidence for accretion found in our data, we are unable to put constraints on the time of accretion.
%Cosmological hydrodynamic simulations show that smooth accretion is the most likely scenario to build gas disks at high redshift (z $\sim$ 1). This form of accretion can provide \HI\ reservoirs of up to 10$^{10}$ \msun\ (Eagle, more recent simulation paper!!!). Our \HI-excess galaxies contain more gas, thus it is likely that additional gas accretion processes, e.g., mergers and gas transfer via galactic winds, contribute as well. 
%{\bf - do the math for Luca's argument -  the outer disks must have been formed in the last XXX Gyrs. }
%{\bf We show that these are LSB galaxies. If angular momentum is high they could have been born in high angular momentum haloes, so they were just slowly evolving. However, this is unlikely given the SFR density vs. large stellar mass. stuff!!! and why these galaxies matter!!!} 

%The available information is not enough to put constraints on the epoch of gas accretion. However, it seems possible that the bulk of the gas has been settled for many Gyr in these galaxies, and they are enriched by gas-rich mergers during their lifetime.

%Given the large gas masses involved, it is likely that not just a single process, but a combination of these enrich the gas reservoirs.

 
%In order to further test the formation scenarios proposed in this paper, \HI-excess galaxies need to be compared to control samples in terms of their \HI\ properties, the presence of low surface brightness outskirts, environment. Such a comparison would shed light on whether \HI-excess galaxies are unique, peculiar objects in terms of their gas accretion processes, or the observed multiwavelength properties are generally found in all types of galaxies. Furthermore, an increase in sample size will allow for a statistical study of the dominant processes responsible for creating \HI-excess galaxies.





%***************************************************************************

%Other \HI-rich galaxy samples exist in the literature focusing on studying the physical processes responsible for the accumulation of large \HI\ reservoirs in galaxies. Samples like Bluedisk \citep{Wang2013}, HIghMass \citep{Huang2014}, \HI\ monsters \citep{Lee2014}, HIGHz \citep{Catinella2015}, and the more recent HIX sample \citep{Lutz2017}, predominantly contain late-type galaxies that are scaled-up versions of star-forming disks. As already discussed in Paper I, the main difference between our \HI-excess galaxies and these \HI-rich samples stands in their selection. The latter analyse the gas content of galaxies compared with their stellar properties (stellar mass, luminosity), which selection preferentially leads to picking star-forming galaxies. On the other hand, our \HI-excess galaxies are selected against high levels of star formation.Another study by \cite{Lemonias2014} has identified a subsample of very massive (log$(M_{\star} / M_{\odot}) > 10.5$), inefficiently star-forming \HI-rich population in the ALFALFA survey. Unlike other \HI-rich samples, these galaxies do not follow the star-forming main sequence in the $M_{\star}$ vs. sSFR (SFR $M_{\star}^{-1}$) relation. Massive, bulge-dominated galaxies are common among this population, thus we expect this sample to be more similar to our \HI-excess selection regarding their formation history. The \cite{Lemonias2014} measurements are represented by green square symbols in Fig. \ref{fig:KS}. As expected, they span a similar region of the Kennicutt-Schmidt relation as our \HI-excess sample. We note that two from the \cite{Lemonias2014} galaxies (GASS 13340 and GASS 45664) are also included in our \HI-excess sample. These galaxies reveal massive bulges and low surface brightness stellar regions in the SDSS images similarly to the sample studied in this paper. A more comprehensive study of these cases will be provided in a future paper.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%We can also test morphological quenching using a different approach. If the presence of a spheroid is responsible for the low star-forming efficiency, then all bulge-dominated galaxies are expected to host low molecular gas fractions. In Fig. \ref{fig:MorphQuench} the molecular gas fraction of the two \HI-excess galaxies with CO observations is compared to the \atlas\ sample (if we want to keep this comparison then I will put in references here). \HI-excess galaxies are located in the low molecular gas fraction regime compared to \atlas\ galaxies in the same stellar mass range. This comparison also shows that the mere presence of a bulge is not enough to shut down star formation in a galaxy, as many bulge-dominated galaxies in \atlas\ do form large amounts of molecular gas. %However, one can find examples for bulge-dominated galaxies with higher molecular gas fractions in the literature. 

%We note that internal dust corrections were not applied in our sample. 
%Except for AGC 192040, all galaxies have an elongated stellar morphology pointing to an inclined view of the disk. In the presence of dust the light has to travel through larger columns of dust in an edge-on disk, and the colours will appear to be redder. Thus the NUV$-r$ colours would become bluer if we corrected for inclination.
% were corrected for internal dust corrections were applied and the galaxies would move even closer to the HIghMass distribution.   
%The difference in gas fractions in Fig. \ref{fig:MorphQuench} (right) is likely due to the fact that the CO in \atlas\ galaxies dominates the central regions of galaxies, whereas the \HI\ in our sample is distributed in extended, low surface density disks. 
%In fact, in our multiwavelength dataset the combination of optical and \HI\ kinematics gives the most clear evidence for gas accretion. Kinematic information will be crucial for identifying 
%We speculate that this galaxy is re-building its disk, where part of the gas has recently (less than an orbital period ago) reached the galaxy at a high angular momentum. This scenario would also explain the exceptionally high gas fraction of this galaxy compared to its stellar mass. 


%The low star-forming efficiency in \atlas\ early-type galaxies is generally attributed to low gas column densities of externally accreted gas.


%{\bf to be worked out once we estimate the Spin parameter !!! - }
%The latter study suggests that high angular momentum is the reason behind the \HI-richness of galaxies with such high gas fractions in the HIX sample, and we discuss this possibility for our sample below.
%compared to early-type galaxies from \atlas, our four \HI-excess galaxies have higher gas fractions, so this is why they are at upper envelope of the mu_star vs. gas fraction relation, they are the most gas-rich systems amongst bulge-dominated galaxies. So how can these galaxies keep such large gas reservoirs?
%Information on the molecular gas content is only available for AGC 192040. 
%surprisingly high for galaxies of >1010 \msun\ stellar mass.
%making it one of the most gas-rich, massive galaxies in the nearby Universe.
%- G20339 has a high gas fraction for its stellar mass, but the other galaxies don’t. This means that they are not particularly \HI-rich for galaxies of the same stellar mass.
%- inefficient star-formers- KS law. CO informations is available for G20339, which has a hard time converting HI into CO. Also in the case of G3505 only an upper limit was found, but we don’t have CO for the other galaxies.



% and prograde rotation of the satellite relative to the central galaxy is known to enhance this effect (Toomre & Toomre 1972). As a result, the gas gets trapped at the outskirts of the massive galaxy in a stable condition, unable to form stars. However, minor mergers can not explain the large gas masses (MHI 􏰀 1010 Modot) detected in H I-excess galaxies, especially in low-density environments where interactions are less likely. 

\subsection{Environment}\label{Sec:env}

It has been known for several decades that high density environments, such as clusters, play a very important role when it comes to gas removal processes \citep{Giovanelli1983, Solanes2001, Catinella2013, Denes2016}. Low-density environments, on the other hand, provide favourable conditions for galaxies to accumulate gas \citep{Wang2015, Janowiecki2017}. In Paper I we show that GASS 3505 lives in a low density environment populated by gas-rich galaxies, the perfect neighbourhood for building and maintaining a large gas reservoir. 
Now we examine the observed volume around the other four \HI-excess galaxies both in \HI\ and in the SDSS spectroscopic catalog. Our sample is selected against \HI\ confusion within the ALFALFA beam, therefore we avoid the densest environments by selection.

We find two galaxies in the vicinity of GASS 20339 with available SDSS spectroscopy, however the galaxies are not detected in \HI\ at the $3\sigma$ upper limit of log$(M_{\rm HI}) < 9.6 $ \msun\ (assuming a line width of 200 \kms). These galaxies are marked as red boxes in Fig. \ref{fig:G20339_env}. The \HI\ non-detections are likely due to the fact that these galaxies are located in high-noise regions of the cube, far away from the phase centre where the sensitivity declines due to the effect of the primary beam.

In the environment of J1126 we find two \HI\ detections with faint optical counterparts in SDSS, see Fig. \ref{fig:J1126_env}. Interestingly, these dwarf galaxies do not have optical spectroscopy, similarly to the cases found in the neighbourhood of GASS 3505. The \HI\ detection of the dwarf in the north is discussed in Sec. \ref{Sec:HIprop}. The second galaxy has an \HI\ mass of log$(M_{\rm HI}) = 9.1$ \msun.  

We also find an \HI\ detection nearby J1558 with SDSS spectroscopy, and we measure its \HI\ mass to be log$(M_{\rm HI}) = 9.7$ \msun. The environment of J1558 is shown in Fig. \ref{fig:J1558_env}.

J1605 does not have any SDSS or \HI-detected neighbours, therefore we do not show a map of this galaxy in the Appendix. 

These examples support the results found for GASS 3505, that \HI-excess galaxies are typically found in low-density environments. Even though we are still limited by number statistics, it appears that optically faint dwarf galaxies are often found in the vicinity of such \HI\ beasts. However, control samples are needed to address whether \HI-excess galaxies are exceptional in this sense, or optically faint companions are typical for all (massive) galaxies. The \HI\ masses detected in dwarf galaxies are too low to push galaxies into the \HI-excess regime once accreted, however these are clearly contributing in some cases. 


   
%\begin{table}
%  \caption{Properties of galaxies in the environment of the \HI-excess sample - {\bf to be completed}. Col.1 SDSS identification number; Col.2 redshift; Col.3 projected distance from the central galaxy; Col.4 stellar mass; Col.5 \HI\ mass}\label{table:summary}
  
%   \begin{center}
%     \begin{tabular}{c c c c c} 		
    %&  & References\\ 	
%\hline									     
%SDSS ID  & z  & $d_{\rm proj}$ & log($M_{\star}$) & log($M_{\rm \HI}$)  \\ 
%         &    &  kpc           &   [\msun]        &  [\msun]            \\
%\hline	
% &  &  &  &   \\ 
%     &  &  &  &  \\
%    &  &  &  &  \\
%    &  &  &  &   \\

%\end{tabular}


    %\begin{tablenotes}
   %  {\bf References.} (1) Catinella et al. (2010); (2) Saintonge et al. (2011a)
    % \item[$\dagger$]  The stellar mass is from SDSS.
    	%\end{tablenotes
%\end{center}
%\end{table}



%- Environment: SDSS images overlayed with detections and non-detections. GASS 20339 has X detected and Y non-detected...The same for the others... Any of these gravitationally bound?
%All isolated centrals in Yang., although we detect a few dwarf galaxies without SDSS spectra, for example near GASS 3505 and J1126. These galaxies live in a low-density environement of gas-rich galaxies, perfect for building and mainting the \HI-excess gas reservoirs.


\section{Introduction}\label{Sec:Intro}

%The difference between our studied \HI-excess galaxies and other \HI-rich samples is that star formation in our sample is a lot more diffuse. 

Numerical simulations predict that cosmic filaments provide fresh supplies of gas that form stars in galaxies at high redshift \citep{Binney2004, Keres2005, Dekel2009}. In the nearby Universe, star-forming galaxies can accrete gas from their halos via the galactic fountain mechanism, furthermore gas-rich mergers and infall from the intergalactic medium can be responsible for supplying fresh gas reservoirs in all galaxies \citep{Sancisi2008}. Once the gas reaches the inner regions of a galaxy and settles into a disk, the signatures of gas accretion (e.g., scattered clouds, streams, tails) will disappear soon after completing 1-2 orbits (equal to a few Gyr for massive galaxies, \citealt{vanWoerden1983, Serra2006}), and the gas will be converted into stars. Given the interplay between gas and star-formation, a well known correlation \citep{Schmidt1959, Kennicutt1989, Kennicutt1998} exists between gas content (either \HI+H$_2$ or H$_2$) and star formation rate (SFR). This is commonly observed in star-forming disks where the density of \HI\ is high enough to be converted into molecular gas. However, this relation breaks down at low gas densities, where star-forming processes are highly inefficient. This is particularly relevant at galaxy outskirts \citep{Bush2008, Leroy2008, Bigiel2010}, where the gravitational potential is very shallow and high angular momentum may restrict the collapse of gas \citep{Kim2013, Obreschkow2016, Lutz2017}. Thus, if the gas is unable to reach the central regions, it will remain preserved in atomic form at the galaxy outskirts, resulting in a disconnection between \HI\ and star-forming properties. 


In our previous work (\citealt{Gereb2016}, Paper I from now on), we identified a rare population of so-called \HI-excess systems, which might be good candidates for galaxies that have recently accreted gas. These are characterised by high gas fractions ($M_{\rm HI}/M_{\star}$) paired with low star-forming efficiencies (estimated based on the combination of NUV$-r$ color and stellar mass surface density, $\mu_{\star}$) in the GASS sample \citep{Catinella2010, Catinella2013}. The prototype galaxy of this class, GASS 3505, was analysed in detail in Paper I. The contrast between its 10$^{9.9}$ \msun\ of \HI\ mass and low level of star formation (0.1 $M_{\odot}$ yr$^{-1}$) pushes GASS 3505 into the \HI-excess regime. We carried out follow-up observations with the Very Large Array (VLA) to map the distribution and kinematics of the \HI\ gas, and identified several signatures suggesting that GASS 3505 has experienced interactions with its environment: a stellar stream in the deep images suggestive of a minor merger; an outer \HI\ ring pointing to external origin of the gas in the interferometric \HI\ observations. 
We carried out numerical simulations and showed that a GASS 3505-type \HI\ ring can be formed in a merger between a gas-rich and a bulge-dominated galaxy. However, GASS 3505 is only one example, and a larger sample needs to be explored in order to understand the \HI-excess population as a whole. 

%Do all \HI-excess galaxies accrete gas through minor, gas-rich merger events?
 %This example shows that multiwavelength, high-resolution observations are the key in identifying the signatures of recent merger/gas accretion events in \HI-excess galaxies. 


We are carrying out an observing campaign with the Giant Metrewave Radio Telescope (GMRT) to image the gas distribution of \HI-excess galaxies. In this paper we present the GMRT observations of four \HI-excess galaxies along with Very Large Telescope (VLT) and Canada France Hawaii Telescope (CFHT) deep optical imaging and Keck spectroscopy from dedicated follow-up observations. In addition to the above, Sloan Digital Sky Survey (SDSS; \citealt{York}) photometry and spectroscopy, furthermore Galaxy Evolution Explorer (GALEX; \citealt{Martin2005}) imaging are also available by selection. 
{\bf These multiwavelength data allow us to explore the \HI-excess in relation to star formation, structure, gas accretion signatures in the sample, and bring us a step closer to understanding the evolutionary processes in these galaxies. }
In this paper the standard cosmological model is used with parameters $\Omega_{\rm M}$ = 0.3, $\Omega_{\Lambda}$ = 0.7 and $H_0$ = 70 km s$^{-1}$ Mpc$^{-1}$. 


\begin{figure}
\includegraphics[width=.5\textwidth]{Plots/GFplane_recalculated.png}
\begin{center}\caption{Gas fraction plane for ALFALFA and GASS galaxies with $M_\star > 10^{10}$ M$_{\odot}$.
Red, empty circles indicate the GASS sample, grey points represent ALFALFA galaxies, and filled red circles show the \HI-excess sample. Green triangles are the GASS upper limits. Star symbols mark the four \HI-excess galaxies studied in this paper. {\bf The coloured star symbols represent the four galaxies with updated NUV$-r$ measurements, as discussed in Sec. \ref{sec:color_mustar}}. The solid line represents the 1:1 relation, and the dashed lines the 2.5$\sigma$ deviation from it. The values of the coefficients are a = -0.240, b = -0.250, c = 2.083.
}\label{fig:GFplane}
\end{center}
\end{figure}


\begin{figure*}
\begin{picture}(600,600)(0,0)
%\graphpaper(-50,-100)(500,700)
%\put(-60,390){\framebox(290,140){}}
\put(-20,475){\includegraphics[width=.22\textwidth]{Plots/SDSS_G20339.png}}
\put(90,460){\includegraphics[width=.9\textwidth]{Plots/Collection_G20339.png}}
\put(-20,320){\includegraphics[width=.22\textwidth]{Plots/SDSS_J1126.png}}
\put(90,310){\includegraphics[width=.9\textwidth]{Plots/Collection_J1126.png}}
\put(-20,175){\includegraphics[width=.22\textwidth]{Plots/SDSS_J1558.png}}
\put(90,160){\includegraphics[width=.9\textwidth]{Plots/Collection_J1558.png}}
\put(-20,20){\includegraphics[width=.22\textwidth]{Plots/SDSS_J1605.png}}
\put(90,10){\includegraphics[width=.9\textwidth]{Plots/Collection_J1605.png}}
\end{picture}
\caption{Multiwavelength observations of the \HI-excess galaxies. From left to right: SDSS optical image, FUV image overlayed with \HI\ contours, \HI\ column density, \HI\ velocity field. {\bf The \HI\ contours range between $3\sigma$ and maximum intensity with steps of a few$\times\sigma$, based on the dynamic range. }} \label{fig:Collection}
\end{figure*}




%Then if you want add a few bits about what these datasets will be used for.
%In this paper we present a larger sample of four \HI-excess galaxies with available multiwavelength observations. 

%In a recent study  we presented a prototype \HI-excess galaxy, GASS 3505, that maintains large gas reservoirs and inefficient star formation activit. huge \HI\ reservoirs (with a mean \HI\ mass of log(M$_{\rm HI}$)$ = 10.1$) and little if any star formation activity, and are identified as being strong outliers in gas fraction vs. color scaling relations.high gas fractions ($M_{\rm HI}/M_{\star}$) paired with low star-forming efficiencies (estimated based on the combination of NUV$-r$ color and stellar mass surface density, $\mu_{\star}$) in the  database.

%- other comments?
%- plots
%- environment check
% A need for on-going gas accretion to the present epoch, which replenishes atomic hydrogen (\HI) consumed by star formation, is well motivated both theoretically and observationally. For example, accretion of gas is invoked to explain the continuous star formation over cosmic times in galaxies like our own Milky Way \citep{Larson1972, Twarog1980, Binney2000}.  
% While testing of the first scenario with observations is very time-expensive \citep{Fraternali2002, Heald2011}, accretion from the external environment can manifest observationally in many ways, i.e., scattered gas clouds, tails, unsettled morphology \citep{Sancisi2008}. {\bf However, the interpretation of these features is limited as gravitational interactions with the environement can also explain the same phenomena. } 



\section{Analysis and Results}\label{Sec:Results}

\subsection{Updated colour and stellar surface density measurements}\label{sec:color_mustar}

%\subsection{Re-measuring the NUV-r colours} 
 %Given the large extent of \HI-excess galaxies (up to 50 arcsec in the SDSS $r$-band images), parts of the outer disks might be missed in the colour measurements. 
%In view of these limitations, 

{\bf
The presence of blue outskirts in \HI-excess galaxies (Fig. \ref{fig:Collection}, left panel) warrant that colour gradients are involved in the modelMag photometry in SDSS\footnote{http://www.sdss3.org/dr8/algorithms/magnitudes.php}. As a result, the measured colour will strongly depend on the used aperture. 
Given that the SDSS measurements are optimised for the central regions where the galaxies are redder, here we re-measure the total NUV$-r$ colour in the four \HI-excess galaxies using large enough apertures that include the total flux. By doing this, we can also test whether the \HI-excess in the gas fraction plane is not due to an aperture effect. 


We define a circular or elliptical region based on the axis ratio and position angle of the galaxies, with a radius that covers the extended outskirts around each galaxy in the GALEX NUV images. We calculate the total magnitude inside these NUV regions both for the NUV\footnote{https://asd.gsfc.nasa.gov/archive/galex/FAQ/counts$\_$background.html} and the SDSS\footnote{http://www.sdss3.org/dr8/algorithms/magnitudes.php} $r$-band images. The colours are corrected for Galactic extinction based on \cite{Wyder2007}. 

The newly measured NUV$-r$ colors are shown as function of gas fraction in Fig. \ref{fig:diagnostics} (left). The previous (catalog-based) measurements of the four galaxies are marked as stars, and the new, total NUV$-r$ measurements are shown as coloured circles. 
The GASS sample is represented by blue shaded regions in these plots, and \HI-excess galaxies are overplotted in red. {\bf We note that the \cite{Brown2015} sample is not shown because the selection of \HI-excess galaxies is solely based on GASS. 
Fig \ref{fig:diagnostics} clearly shows that \HI-excess galaxies occupy a different region than GASS in the log($M_{\rm HI}/M_{\star}$) vs. NUV$-r$ plane. 
The four \HI-excess galaxies analysed in this paper move bluewards after we include the outskirts.
However, the galaxies remain at the upper envelope of the colour vs. gas fraction relation. We also show the new location of the galaxies in the gas fraction plane, marked as coloured circles in Fig. \ref{fig:GFplane}. The galaxies move closer to the plane, however the \HI-excess is still $>2.5\sigma$ even after we include the contribution of the bluer disks. }


Exclusion of outer disks can also contribute to the overestimation of the stellar surface density in galaxies. The SDSS Petrosian $r_{50,z}$ radii in the $z$ filter (used to compute $\mu_{\star}$ values in Fig. \ref{fig:GFplane}) range between 1-5 arcsec in the four galaxies, however the low surface brightness disks are a few$\times$10 arcsec in size. In fact, the $z$-band filter is not sensitive enough to detect these faint outskirts at its 20.5 mag limit.
The highest signal-to-noise ratio in SDSS is measured in the $r$-band, with a sensitivity limit of 22.2 mag.
In the following we use the more sensitive SDSS $r$-band images to measure the $r_{\rm eff}$ (the radius at which half of the total light is emitted), and re-calculate the $\mu_{\star, r}$ in the selected sample. 
We note that even though deep imaging is available for three out of four galaxies, these are taken in different bands and there is no comparison sample available. 


The $r_{\rm eff}$ is measured in the four galaxies based on the curve of growth method following the technique applied in SDSS. We define circular apertures around the centre of the galaxies using the $r$-band images, where the $r_{\rm eff}$ corresponds to the radius of the aperture containing half of the total flux.
For consistency, the stellar mass density is re-calculated for the entire sample using catalog-based $r$-band measurements, such as $\mu_{\star}$ = $M_\star$ /(2$\pi$ $r_{50,r}^2$), where $r_{50,r}$ is the radius containing 50$\%$ of the Petrosian flux in the SDSS $r$-band in DR7.
The $\mu_{\star}$ measurements are shown as function of gas fraction in Fig. \ref{fig:diagnostics} (right).
The $\mu_{\star}$ values of the four galaxies based on the SDSS Petrosian $r_{50,r}$ are shown as stars, and we also show the new measurements based on $r_{\rm eff}$ marked as coloured circles. GASS and \HI-excess galaxies are marked as blue shaded regions and red points, respectively. We note that the difference in SDSS $r$-band and $z$-band Petrosian radius is less than 1 arcsec in about 90$\%$ of the sample, thus this plot shows the same trends when using the $z$-band radii.
Three out of the four galaxies analysed in this paper are clear outliers (star symbols) in Fig. \ref{fig:diagnostics} (right), however they move closer to the GASS distribution after the outskirts are accounted for (coloured circles). The $r_{\rm eff}$ shows a dramatic change in the case of AGC 192040, from a Petrosian $r_{50,z}$ = 1.45 arcsec to $r_{\rm eff}$ = 11 arcsec (with an error of 3 arcsec). The $r_{\rm eff}$ radius of the other three galaxies is up to 2.5 times larger than their Petrosian $r_{50,z}$. The galaxies are not that extreme anymore based on the new $r$-band measurements, but they are still located at the upper envelope of the $\mu_{\star}$ vs. gas fraction relation. It is clear that the four \HI-excess galaxies are among the most gas-rich galaxies for their structure even after we include the outskirts.

For AGC 192040 we also see a clear segregation of the bulge and an extended disk component in the $r$-band image, and find that the SDSS magnitude measurements are mainly confined to its bulge. This suggest that the total stellar mass of the galaxy is underestimated. 
We measure the total flux of the galaxy and estimate the stellar mass of the disk based on the difference between the total and bulge magnitude. The outer disk represents only $\sim5\%$ of the bulge mass, showing that most of the total stellar mass is contained in the centre. We note that the position of the blue circle in Fig. \ref{fig:diagnostics} (right) is based on this updated stellar mass. For the other galaxies the bulges and disks are not well defined, thus bulge-disk decomposition would be needed to measure the different components independently. 

When we compare the two panels in Fig. \ref{fig:diagnostics}, \HI-excess galaxies (red points) are stronger outliers compared to the GASS sample in the NUV$-r$ vs. gas fraction relation, and they have a larger overlap with the underlying distribution in terms of their $\mu_{\star}$.
This suggests that colour is the main reason behind the \HI-excess selection in the gas fraction plane, but galaxy structure plays a secondary role.

%Outliers are present in Fig. \ref{fig:diagnostics} (right) as well, suggesting that 
}

%\begin{figure*}
%\includegraphics[width=.9\textwidth]{Plots/Collection_G20339.png}
%\includegraphics[width=.9\textwidth]{Plots/Collection_J1126.png}
%\includegraphics[width=.9\textwidth]{Plots/Collection_J1558.png}
%\includegraphics[width=.9\textwidth]{Plots/Collection_J1605.png}
%\begin{center}\caption{Multiwavelength observations of the \HI-excess galaxies. From left to right: FUV image overlayed with \HI\ contours, \HI\ column density, \HI\ velocity field.} \label{fig:Collection}
%\end{center}
%\end{figure*}


%\newpage
%\pagestyle{empty}

%From the top to the bottom the galaxies are: AGC 192040, AGC 731712, AGC 10111, AGC 263047.}



%The NUV$-r$ colours are estimated based on the GALEX NUV and SDSS $r$-band images.

\subsection{Signatures of accretion in the multiwavelength data}\label{sec:multiwavelength}
 
In this Section we explore the sample through our multiwavelength observations and look for signatures of gas accretion as a source for the gas excess in the \HI-excess sample.
%{\bf to see if we can find signatures of gas accretion that can explain the gas excess. }
%to look for signatures that can explain the presence of excess \HI\ gas in these galaxies, for example gas accretion.

Figures \ref{fig:Collection} and \ref{fig:Collection_Optical} give an overview of the optical, UV and \HI\ properties of the sample. Deep optical imaging in Fig. \ref{fig:Collection_Optical} shows that a common feature of our \HI-excess galaxies is $\gtrsim$24 mag arcsec$^{-2}$ surface brightness stellar regions extending to large radii (up to 70 kpc radius in AGC 192040).
These are typical surface brightnesses for the diffuse light measured at the outskirts of galaxies where tidal streams and shells are often created as a result of galaxy interactions and mergers \citep{Janowiecki2010, Martinez2010, Duc2015}. The faint regions in Fig. \ref{fig:Collection_Optical} do not reveal shells or obvious stellar streams, instead they are distributed in spiral arms. The FUV images in Fig. \ref{fig:Collection} (second to left panel) support the presence of star-forming regions, where star-formation is embedded in \HI\ gas as indicated by the contours (in black).


We identify a stellar tail in the VLT image of AGC 192040 (see Fig. \ref{fig:Collection_Optical}), coinciding with an \HI\ cloud detached from its main body of rotation (see red ellipse in the position-velocity diagram in Fig. \ref{fig:HI_pv_cloud}). 
Similar features are present in M 101 \citep{Hulst1988} and NGC 262 \citep{Simkin1987}, and these structures are thought to have formed through minor mergers (see more examples in \citealt{Sancisi2008}). {\bf Following these examples, the \HI\ tail in AGC 192040 is likely to be a tidal stream caused by galaxy interactions.} We note that this cloud of gas contributes $\sim15\%$ to the \HI\ mass, and AGC 192040 remains an \HI-excess galaxy even when we exclude this gas mass from our calculations. There is no clear trace of similar tidal tails in the other three \HI-excess galaxies. 

%This example shows that the advantage of \HI\ compared to deep imaging stands in its ability to both map the gas and measure its kinematics.


Fig. \ref{fig:Collection} (right panel) presents the velocity field and Fig. \ref{fig:HI_pv} the position-velocity measurements of the \HI\ gas. 
{\bf In Fig. \ref{fig:HI_pv} we also show the Keck measurements, where nebular emission lines arise due to the presence of ionized gas (cyan points) and absorption lines are coming from stellar photospheres (red points).
} The agreement between the ionised and \HI\ gas kinematics suggests that these two gas phases are part of the same structure. The bulk of the gas is in a rotating configuration in all galaxies. However, the position-velocity diagram of AGC 10111 suggests that the stars in the central bulge are counter-rotating with respect to the ionised/\HI\ disk. We measure the counter-rotation to be statistically significant by comparing the amplitude of the slope to the uncertainties from the Gaussian fits to absorption lines. Counter rotation is a strong indication that AGC 10111 {\bf has externally accreted some gas}.  

{\bf In summary, AGC 10111 is the only galaxy in our sample showing clear signatures of gas accretion in form of counter-rotation. The gas kinematics in AGC 192040 is suggestive of a recent interaction, however based on the data it is not clear if the galaxy is in the process of swallowing a companion, or the disturbance is due to tidal interactions. No obvious evidence for gas accretion is found in the other galaxies. }

%a good candidate for going through a gas-rich, minor merger event, however it is not clear 
%is a lower limit as not all gas accretion events result in counter-rotation. AGC 192040 is a good example for a galaxy that is going through a gas-rich, minor merger as indicated by the combination of deep optical imaging and \HI\ kinematics. Thus, in our sample 50$\%$ (two out of four) of the galaxies reveal prominent gas accretion signatures.
%It is worth mentioning that the other two galaxies also show indirect signatures of gas accretion, e.g., warps. 
%in two cases (AGC 731712 and AGC 263047). Numerical simulations show that warps can be created when gas is accreted onto the disk with a slewed angular momentum in galaxies like the Milky Way \citep{Ostriker1989, Jiang1999}. However, tidal interactions can also cause disks to warp in denser environments. In Sec. \ref{Sec:env} we study the environment of the four \HI-excess galaxies to test the viability of these scenarios, and we discuss our results in Sec. \ref{Sec:Discussion}.
%In our dataset the combination of optical and \HI\ kinematics gives the most clear evidence for gas accretion in form of counter-rotation in one galaxy. However, 


\begin{figure*}
\begin{center}
\includegraphics[width=.45\textwidth]{Plots/MHI_Color.png}
\includegraphics[width=.45\textwidth]{Plots/MHI_mustar.png}
\caption{Left panel: \HI\ gas fraction ($M_{\rm HI}/M_{\star}$ ) vs. NUV$-r$ colour relation of \HI-excess galaxies (red points). The blue shaded region marks the GASS sample. \HI-excess galaxies studied in this paper are shown as coloured stars. Right panel: \HI\ gas fraction vs. stellar mass surface density ($\mu_{\star}$) for the same samples.}
\label{fig:diagnostics}
\end{center}
\end{figure*}



\begin{table*}
  \caption{Basic properties of the \HI-excess galaxies. Col.1 name used in this paper; Col.2 right ascension; Col.3 declination; Col.4 redshift; Col.5 stellar mass surface density measured from SDSS; Col.6 NUV-r color based on GALEX and SDSS measurements; Col.7; Stellar mass ; Col.8 Arecibo \HI\ mass; Col.9 global SFR measured within the FUV radius, see Sec. \ref{Sec:UVprop} for details.}\label{table:summary}
  
   \begin{center}
     \begin{tabular}{c c c c c c c c c}		
    %&  & References\\ 	
\hline									     
Name &  RA   & Dec   & z & log($\mu _{\star}$)      & NUV $-$ $r$ & log($M_{\star}$) & log($M_{\rm \HI}$)  & SFR \\ 
     & [deg] & [deg] &   & [M$_{\odot}$ kpc$^{-2}$] & [mag]       &   [\msun]        &  [\msun]            &  [\msun yr$^{-1}$] \\
\hline	
AGC 192040  & 09:47:32.79   & +10:45:08.72  & 0.047  & 9.4  & 2.23  & 10.54  & 10.76  & 0.92  \\ 
AGC 731712  & 11:26:50.06   & +24:04:52.89  & 0.025  & 9.26 & 3.89  & 10.16  & 10.12  & 0.24 \\
AGC 10111   & 15:58:13.16   & +13:10:07.80  & 0.035  & 9.38 & 4.12  & 10.32  & 10.23  & 0.14 \\
AGC 263047  & 16:05:01.53   & +26:07:15.03  & 0.026  & 8.44 & 3.92  & 10.03  & 10.08  & 0.05 \\
\hline
\end{tabular}
    %\begin{tablenotes}
   %  {\bf References.} (1) Catinella et al. (2010); (2) Saintonge et al. (2011a)
    % \item[$\dagger$]  The stellar mass is from SDSS.
    	%\end{tablenotes
\end{center}
\end{table*}


\subsection{Star-forming properties of the \HI-excess sample}\label{Sec:UVprop}

In Paper I we showed that the star-forming processes in GASS 3505 are very inefficient, with gas depletion timescales of $\sim10^{11}$ yr. Such long timescales are typical for galaxy outskirts in general, where the column density of \HI\ is low \citep{Bigiel2010}. In AGC 192040, \cite{Lee2014} carried out molecular gas observations and detected log$(M_{\rm H2})$ = 9.37 \msun, which translates into a molecular gas fraction of log($M_{\rm H2} /M_{HI}$) = -1.39. This number is very low compared to the COLD GASS distribution, where the average molecular gas fraction for a massive galaxy like AGC 192040 is log($M_{\rm H2} /M_{HI}$) = -0.5, suggesting that molecular gas formation is a very inefficient process in this galaxy. The other three galaxies in our sample do not have molecular observations available. 


FUV emission is present in all galaxies in Fig. \ref{fig:Collection} (second to left panel), coinciding with the highest column density \HI\ regions. We measure the SFR vs. \HI\ surface density relation (also known as the Kennicutt-Schmidt relation, \citealt{Schmidt1959, Kennicutt1989, Kennicutt1998}) in each pixel of the maps to learn about the efficiency of star formation in the \HI-excess sample.  Star-forming regions (where the FUV flux is higher than $3\sigma$) are marked as filled circles, upper limits (where the FUV flux is lower than $3\sigma$) as triangles in Fig. \ref{fig:KS}. Star symbols mark the global measurements estimated within the FUV radius. The corresponding SFR-s are reported in Table \ref{table:summary}. The difference between the $\Sigma_{SFR}$ upper limits of the new sample and GASS 3505 are due to selection. GASS 3505 is from the Medium Imaging Survey (MIS), however for the four new galaxies only shallower AIS maps are available. We also show the measurements by \cite{Bigiel2010} for the outskirts of spiral and dwarf galaxies, {\bf marked as grey circles}. \HI-excess galaxies follow the underlying distribution of galaxy outskirts, revealing inefficiently star-forming regions. Unlike GASS 3505, the new galaxies lie on the higher end of the \HI\ and SFR surface density distribution.  This is not surprising given that the newly selected galaxies all show blue outskirts in SDSS as opposed to GASS 3505.
The gas depletion timescales are between $10^{10} -10^{11}$ year as indicated by the dashed lines.
%Even though the \HI-excess population is a mixed bag in terms of their optical/\HI\ properties, they share similar properties when it comes to their ability to form stars.



\subsection{The environment of HI-excess galaxies}\label{Sec:env}

It has been known for several decades that high density environments, such as clusters, play a very important role when it comes to gas removal processes \citep{Giovanelli1983, Solanes2001, Catinella2013, Denes2016}. Low-density environments, on the other hand, provide favourable conditions for galaxies to accumulate gas \citep{Wang2015, Janowiecki2017}. Now we examine the observed volume around the other four \HI-excess galaxies both in \HI\ and in the SDSS spectroscopic catalog. Our sample is selected against \HI\ confusion within the Arecibo beam, therefore we avoid the densest environments by selection.

The optical and \HI\ maps of the environment are shown in Fig. \ref{fig:G20339_env} - \ref{fig:J1558_env}. 
All galaxies have a few neighbours except for AGC 263047, thus we do not show a map of this galaxy in the Appendix. 
There are two galaxies in the vicinity of AGC 192040 (marked as red boxes in Fig. \ref{fig:G20339_env}) with available SDSS spectroscopy, however these are not detected in {\bf the GMRT \HI\ observations} at the $3\sigma$ upper limit of log$(M_{\rm HI}) < 9.6$ \msun\ {\bf and log$(M_{\rm HI}) < 9.4$ \msun\ } (assuming a line width of 200 \kms). 
The \HI\ non-detections are likely due to the fact that these galaxies are located in high-noise regions of the cube, far away from the phase centre where the sensitivity declines due to the effect of the primary beam.
In the environment of AGC 731712 we find two \HI\ detections with faint optical counterparts in SDSS. These dwarf galaxies do not have optical spectroscopy, similarly to the cases found in the neighbourhood of GASS 3505. We also find an \HI\ detection nearby AGC 10111 with available SDSS spectroscopy. The properties of these galaxies are summarized in Table \ref{table:appendix}.

In the following analysis we explore whether the neighbours are gravitationally bound to the \HI-excess galaxies. A system is considered gravitationally bound if its potential energy exceeds the total kinetic energy, i.e., if $(G \times M)/r_{\rm sep} > 1/2 \times v^{2}$, where $G$ is the gravitational constant, $M$ is the total mass of the system, $r_{\rm sep}$ is the physical separation between the pair of galaxies, and $v$ is the velocity difference between these two \citep{Evslin2014}. The three-dimensional velocity field can be approximated as $v \simeq \sqrt{3} v_{\rm los}$ for an isotropic system, where $v_{\rm los}$ is the line-of-sight velocity difference.{\bf The parameters used in these calculations are presented in Table \ref{table:appendix}}. The total mass of every pair is calculated as the sum of $M_{\rm halo} + M_{\star} + M_{\rm HI}$, where $M_{\rm halo}$ is estimated using the stellar mass based on a study by \cite{Behroozi2013}.
In the last column of Table \ref{table:summary} we present the outcome of this analysis marking gravitationally bound galaxies with $1$, and non-members with $0$. We find that two of the neighbouring galaxies are gravitationally bound, however three other cases are not associated to \HI-excess galaxies. 
These examples support the results found for GASS 3505, that \HI-excess galaxies are typically found in low-density environments, i.e., in small groups or in isolation. Such environments are perfect for galaxies to build and preserve \HI-excess gas reservoirs.


\begin{figure}
\includegraphics[width=.43\textwidth]{Plots/PV_G20339_cloud.png}
\begin{center}\caption{\HI\ position-velocity diagram of AGC 192040 extracted along PA = 78.4 deg.
 The red ellipse marks the location of the \HI\ tail.} \label{fig:HI_pv_cloud}
\end{center}
\end{figure}


\begin{figure}
\includegraphics[width=.45\textwidth]{Plots/K_S.png}
\begin{center}\caption{SFR surface density vs. \HI\ surface density relation at the low end of the Kennicutt-Schmidt law. Star-forming regions in \HI-excess galaxies (where the FUV emission is above 3$\sigma$) are shown as colored dots, and triangles mark the 3$\sigma$ FUV upper limits. Star symbols mark the global measurements. The Bigiel et al. (2010) and Lemonias et al. (2014) samples are shown in grey points and green squares, respectively. The black dashed lines mark constant gas depletion timescales of 10$^9 - 10^{12}$ yr.}\label{fig:KS}
\end{center}
\end{figure}

%These are typical surface brightnesses for the diffuse light measured at the outskirts of galaxies  
%We calculate the face-on surface brightness at the half-light radius in the SDSS $r$-band images, $\mu_{e}(r)$ in order to quantify whether our \HI-excess galaxies are part of the LSB population. Following \cite{Blanton2005}, we adopt a 23.5 mag arcsec$^{-2}$ cut for the selection, where LSB galaxies are classified to be fainter than this limit. !!!An inclination correction is applied based on ??? (minor-to-major axis ratio?) to achieve the face-on deprojection of the surface brightness!!!. The results are shown in Fig. X, where the vertical dashed line marks the 23.5 mag arcsec$^{-2}$ limit by \cite{Blanton2005}.}The FUV images in Fig. \ref{fig:Collection} (left panel) suggest the presence of star-forming regions at these faint outskirts, where star-formation is embedded in \HI\ gas as indicated by the contours (in black). 

%Thus, deep imaging does not provide evidence for external accretion in this small sample.
%do not reveal shells or obvious stellar streams, instead 
%where tidal streams and shells are often created as a result of galaxy interactions and mergers
%The faint regions (see Fig. \ref{fig:Collection_Optical}) are distributed in spiral arms {\bf and ring-like structures}.
%Blue spiral arms are visible out to xxx r$_{eff}$ in AGC 192040. The other galaxies are less extreme, the outer disk sizes based on the SDSS images are XXX r$_{eff}$, XXX r$_{eff}$, XXX r$_{eff}$ in J1126, J1558, and J1605, respectively.
%The de Vaucouleurs profile used in SDSS is truncated to go to zero at 8$_{eff}$ (the exponential profile at 4$_{eff}$). Thus, parts of the outer disks in \HI-excess galaxies might be missed in the colour measurements, particularly in the case of AGC 192040. 
%In the left panel of Fig \ref{fig:diagnostics} we explore the relation between  NUV$-r$ color and \HI\ gas fraction. 
%******* rewrite.

%\subsection{Remeasuring the Re-measuring the NUV-r colours} 


\section{Sample Selection}\label{Sec:SampleSelection}

Our sample is selected from the GALEX Arecibo SDSS Survey (GASS, \citealt{Catinella2010, Catinella2013}) based on the gas fraction plane, a relation between the measured \HI\ gas fraction and that predicted from the combination of NUV$-r$ color (a proxy for specific SFR) and stellar mass surface density ($\mu_{\star}$, indicator of morphological type), as shown in Fig. \ref{fig:GFplane}. %GASS 3505 is the most extreme outlier within the GASS sample with $>2.5 \sigma$ deviation from the one-to-one relation in this plane, meaning that it has a large \HI\ content with little associated star-formation activity. 

In order to maximise the number of \HI-excess galaxies, which are rare but very \HI-rich, here we combine GASS with the sample of \cite{Brown2015}. From the GASS sample we selected all the galaxies with a gas fraction in excess of $2.5{\sigma}$ from the average relation in Fig. \ref{fig:GFplane}, and examined the SDSS images of each of them to exclude those affected by \HI\ confusion within the 3 arcmin beam of the Arecibo telescope (shown as grey points above the dashed line in Fig. \ref{fig:GFplane}). This yields 36 galaxies. The \cite{Brown2015} sample is extracted from SDSS and cross-matched with the $\alpha.70$ source catalog from ALFALFA, and contains $\sim11230$ stellar-mass selected galaxies restricted to the GASS volume ($0.025 < z < 0.05$, $M_{\star} > 10^{10} M_{\odot}$). From this sample we selected \HI-excess systems not already included in GASS and excluded confused ones, obtaining 28 additional galaxies. Thus, our \HI-excess sample includes a total of 64 galaxies. 


For both samples the stellar masses are taken from the MPA/JHU value added catalogs, based on SDSS DR7\footnote{http://www.mpa-garching.mpg.de/SDSS/DR7/}. The stellar mass surface density is defined as $\mu_{\star}$ = $M_\star$ /(2$\pi$ $r_{50,z}^2$), where $r_{50,z}$ is the radius containing 50$\%$ of the Petrosian flux in the SDSS $z$ band. We note however that the GALEX UV photometry for GASS was reprocessed as in Wang et al (2010), whereas the \cite{Brown2015} sample is taken from the GALEX Unique Source Catalogues\footnote{http://archive.stsci.edu/prepds/gcat/} (GCAT, \citealt{Seibert2012}) and the \cite{Bianchi2014} catalog of Unique GALEX Sources\footnote{http://archive.stsci.edu/prepds/bcscat/} (BCS).
For more details on the sample descriptions see \cite{Catinella2010} and \cite{Brown2015}.

%Galaxies that are confused within the Arecibo beam (grey dots above the $2.5\sigma$ line) are removed from the sample.

The 64 \HI-excess galaxies above the $2.5\sigma$ line are marked in red in Fig. \ref{fig:GFplane}. In this paper we focus on the detailed analysis of four targets marked with coloured star symbols.
These are selected to show signatures of recent star formation, i.e., low surface brightness arms, disks in the SDSS images for optical spectroscopic observation purposes, see left panel of Fig. \ref{fig:Collection}. 
The galaxies are identified by their Arecibo General Catalog (AGC, maintained by M.P. Haynes and R. Giovanelli at Cornell University) number, and their main properties are summarized in Table \ref{table:summary}. 

In what follows, we take advantage of our deep optical, GMRT and Keck follow-up observations to shed light on the physical processes that are responsible for the presence of excess \HI\ gas in these galaxies.

%panel of Fig. \ref{fig:diagnostics}
% In general Bulge -disk decomposition would be needed.

%However, one can identify outliers in the log($M_{\rm HI}/M_{\star}$) vs. $\mu_{\star}$ relation as well.
%Three out of the four new \HI-excess targets (marked as coloured stars) have extreme $\mu_{\star}$ for their gas content in Fig \ref{fig:diagnostics} (right panel). 
% This plot the aperture-corrected $\mu_{\star}$ has decreased in the four galaxies.  
%However, 
%The catalog-based measurements of the 

  %thus based on the presence of outer stellar regions in the SDSS images we need to account for these extended disks.
%Thus, we use the $r$-band images to re-measure the effective radius ($R_{\rm eff}$) for each galaxy. 
%Given the large extent of the disk in AGC 192040, the SDSS magnitude is almost purely confined to the bulge we also calculate the stellar mass of the outer disk.  
% The new measuruments are shown in Fig. \ref{fig:diagnostics} (right).
%marked as coloured circles 
%The $\mu_{\star}$ values used in Fig. \ref{fig:GFplane} are computed based on 
%AGC 192040 has the most prominent disk found in the sample in terms of its gas fraction (XXX) and radius (XXX). Thus, 
%being underestimated

 %we estimate 

 %(). 
 %the we re-calculate the stellar surface density of the four \HI-excess galaxies based on the more sensitive $r$-band observations. 
%where the low surface brightness blue outer disks are not detected. Hence, these regions do not contribute to the measurement. A nice example is AGC 192040, which has a very blue NUV$-r = 2.23$ colour due to its star-forming outskirts, and it falls on the gas fraction vs. colour relation in Fig. \ref{fig:diagnostics} (left). However, this galaxy is the most extreme outlier in the log($M_{\rm HI}/M_{\star}$) vs. $\mu_{\star}$ relation.}
%The presence of outliers in this relation suggest that even though classification as an \HI-excess galaxy is more dependent on (the lack of) star-formation in our sample, galaxy structure plays a secondary role {\bf in the selection. 

%These are rare galaxies where the dominant stellar population (a big red central bulge) is disconnected from the gas (diffuse, extended disk). 
 
%n what follows, we take advantage of our deep optical, GMRT and Keck follow-up observations to shed light on the physical processes that are responsible for the presence of excess \HI\ gas in these galaxies. 


 %whereas the sample has a larger overlap with GASS when it comes to $\mu_{\star}$.
%This suggests that colour is more closely related to their \HI-excess nature than morphology as red points are outliers already in this plane. 

%In other words, the galaxies are {\bf "too red", emphasising again that star formation rate (SFR) in most of the galaxies is inefficient despite the presence of large gas reservoirs. }

%The righ hand panel shows the same relation for $\mu_{\star}$. The goal of this exercise is to determine whether the observed \HI-excess in our sample is more dependent on colour or on $\mu_{\star}$, given that the x-axis of the gas fraction plane uses the combination of these two parameters.


%Given that our \HI-excess galaxies all display faint, star-forming outskirts that were not taken into account for the measurement of their NUV$-r$ colour and $\mu_{\star}$ stellar surface density, here we re-measure these parameters by including the extended disks.

%We define a circular or elliptical region that encompasses the extended outskirts around each galaxy in the GALEX NUV images, and calculate the total magnitude inside these regions both for the NUV\footnote{https://asd.gsfc.nasa.gov/archive/galex/FAQ/counts$\_$background.html} and the SDSS\footnote{http://www.sdss3.org/dr8/algorithms/magnitudes.php} $r$-band images. The colours are corrected for Galactic extinction based on \cite{Wyder2007}. The new NUV$-r$ measurements are marked as coloured circles in Fig. \ref{fig:diagnostics} (left). The points move bluewards as expected, however the galaxies remain at the upper envelope of the colour vs. gas fraction relation. We also show the location of the galaxies in the gas fraction plane (see Fig. \ref{fig:GFplane}) using the new measurements, marked as coloured circles again. The galaxies move closer to the plane, however the \HI-excess is still $>2.5\sigma$ even after we include the contribution of the bluer disks. 

%Fig. \ref{fig:diagnostics} (right) when 
%our selected galaxies are extreme outliers in the $\mu_{\star}$ vs. gas fraction relation, is measured in the SDSS $z$-band, are not sensitive enough for the outer disks to be detected and thus the mu_

%Given that the $\mu_{\star}$ is overestimated when using SDSS $z$-band measurements, we re-calculate the stellar surface density of the four \HI-excess galaxies based on more sensitive observations. 
%Even though deep imaging is available for three out of four galaxies, these are taken in different bands and there is no comparison sample available. Thus, we use the SDSS r-band images and re-measure the effective radius ($R_{\rm eff}$) for each galaxy. This is done based on the curve of growth method following the technique applied in SDSS. We define circular apertures around the centre of the galaxies, where the $R_{\rm eff}$ corresponds to the radius of the aperture containing half of the total flux.
%For AGC 192040 we also calculate the stellar mass of the outer disk. Based on the difference between total magnitude and that of the bulge, we estimate that the outer disk contains $\sim5\%$ of the bulge mass. For the other galaxies the bulges and disks are not well segragated, thus bulge-disk decomposition would be needed to measure the different components independently. The new measurements are marked as coloured circles in Fig. \ref{fig:diagnostics} (right). For consistency, the stellar mass density is re-calculated for the entire GASS and \HI-excess sample such as $\mu_{\star}$ = $M_\star$ /(2$\pi$ $r_{50,r}^2$), where $r_{50,r}$ is the radius containing 50$\%$ of the Petrosian flux in the SDSS $r$-band in DR7. These measurements are presented in Fig. \ref{fig:diagnostics} (right), marked as blue shaded regions and red points for GASS and \HI-excess galaxies, respectively. We note that the SDSS $r$-band and $z$-band petrosian radius is not more than a few arcsec in general, thus these samples do not change much. 






\section{Bibliography}\label{Sec:biblio}


\begin{thebibliography}{Balcells1990}

%\bibitem[\protect\citeauthoryear{Abazajian et al.}{2009}]{Abazajian2009} Abazajian K.~N., et al., 2009, ApJS, 182, 543-558 

%\bibitem[\protect\citeauthoryear{Adelman-McCarthy et al.}{2008}]{Adelman2008} Adelman-McCarthy J.~K., et al., 2008, ApJS, 175, 297-313 

\bibitem[\protect\citeauthoryear{Ahn et al.}{2012}]{Ahn2012} Ahn C.~P., et al., 2012, ApJS, 203, 21 


%\bibitem[\protect\citeauthoryear{Balcells $\&$ Quinn}{1990}]{Balcells1990} Balcells M., Quinn P.~J., 1990, ApJ, 361, 381 

%\bibitem[\protect\citeauthoryear{Balcells et al.}{2001}]{Balcells2001} Balcells M., van Gorkom J.~H., Sancisi R., 
%del Burgo C., 2001, AJ, 122, 1758 

\bibitem[\protect\citeauthoryear{Barnes}{2002}]{Barnes2002} Barnes J.~E., 2002, MNRAS, 333, 481 


\bibitem[\protect\citeauthoryear{Bassett et al.}{2017}]{bassett17c} Bassett R., Bekki K., Cortese L., Couch W.~J., 2017, arXiv, arXiv:1704.08434 


\bibitem[\protect\citeauthoryear{Bekki}{1998}]{Bekki1998} Bekki K., 1998, ApJ, 499, 635 


%\bibitem[\protect\citeauthoryear{Bekki}{2013}]{Bekki2013} Bekki K., 2013, MNRAS, 432, 2298 


%\bibitem[\protect\citeauthoryear{Bertin et al.}{2002}]{Bertin2002}  Bertin E., Mellier Y., Radovich M., Missonnier G., Didelon P., Morin B., 2002, ASPC, 281, 228 


\bibitem[\protect\citeauthoryear{Bianchi, Conti, \& Shiao}{2014}]{Bianchi2014} Bianchi L., Conti A., Shiao B., 2014, AdSpR, 53, 900 


\bibitem[\protect\citeauthoryear{Bigiel et al.}{2010}]{Bigiel2010} Bigiel F., Leroy A., Walter F., Blitz L., Brinks E., de Blok W.~J.~G., 
Madore B., 2010, AJ, 140, 1194 

%\bibitem[\protect\citeauthoryear{1987}]{Binney1987} 1987, Natur, 326, 219 


%\bibitem[\protect\citeauthoryear{Binney, Dehnen, \& Bertelli}{2000}]{Binney2000} Binney J., Dehnen W., Bertelli G., 2000, MNRAS, 318, 658 

\bibitem[\protect\citeauthoryear{Binney}{2004}]{Binney2004} Binney 
J., 2004, MNRAS, 347, 1093 

%\bibitem[\protect\citeauthoryear{Blanton et al.}{2005}]{Blanton2005} Blanton M.~R., Lupton R.~H., Schlegel D.~J., Strauss M.~A., Brinkmann J., Fukugita M., %Loveday J., 2005, ApJ, 631, 208 

%\bibitem[\protect\citeauthoryear{Blanton \& Moustakas}{2009}]{Blanton2009} Blanton M.~R., Moustakas J., 2009, ARA\&A, 47, 159 

\bibitem[\protect\citeauthoryear{Behroozi, Wechsler, \& Conroy}{2013}]{Behroozi2013} Behroozi P.~S., Wechsler R.~H., Conroy C., 2013, ApJ, 770, 57 

\bibitem[\protect\citeauthoryear{Bell et al.}{2004}]{Bell2004} Bell E.~F., et al., 2004, ApJ, 608, 752 


%\bibitem[\protect\citeauthoryear{Booth et al.}{2009}]{Booth2009}  Booth R.~S., de Blok W.~J.~G., Jonas J.~L., Fanaroff B., 2009, arXiv, arXiv:0910.2935 

\bibitem[\protect\citeauthoryear{Boissier \& Prantzos}{2000}]{Boissier2000} Boissier S., Prantzos N., 2000, MNRAS, 312, 398 

\bibitem[\protect\citeauthoryear{Boissier et al.}{2016}]{Boissier2016} Boissier S., et al., 2016, A\&A, 593, A126 


\bibitem[\protect\citeauthoryear{Brown et al.}{2015}]{Brown2015} 
Brown T., Catinella B., Cortese L., Kilborn V., Haynes M.~P., Giovanelli 
R., 2015, MNRAS, 452, 2479 

%\bibitem[\protect\citeauthoryear{Brown et al.}{2017}]{Brown2017} Brown T., et al., 2017, MNRAS, 466, 1275 

\bibitem[\protect\citeauthoryear{Bush et al.}{2008}]{Bush2008} Bush S.~J., Cox T.~J., Hernquist L., Thilker D., Younger J.~D., 2008, ApJ, 683, L13 


%\bibitem[\protect\citeauthoryear{Catinella et al.}{2008}]{Catinella2008} Catinella B., Haynes M.~P., Giovanelli R., Gardner J.~P., Connolly A.~J., 2008, ApJ, 685, L13 


\bibitem[\protect\citeauthoryear{Catinella et 
al.}{2010}]{Catinella2010} Catinella B., et al., 2010, MNRAS, 403, 
683 

\bibitem[\protect\citeauthoryear{Catinella et 
al.}{2013}]{Catinella2013} Catinella B., et al., 2013, MNRAS, 436, 34 

%\bibitem[\protect\citeauthoryear{Catinella  \& Cortese}{2015}]{Catinella2015} Catinella B., Cortese L., 2015, MNRAS, 446, 3526 

%\bibitem[\protect\citeauthoryear{Chabrier}{2003}]{Chabrier2003}  Chabrier G., 2003, PASP, 115, 763 

%\bibitem[\protect\citeauthoryear{Churchill, Steidel, \& Kacprzak}{2005}]{Churchill2005} Churchill C., Steidel C., Kacprzak G., 2005, ASPC, 331, 387 

%\bibitem[\protect\citeauthoryear{Cormier et al.}{2016}]{Cormier2016} Cormier D., et al., 2016, MNRAS, 463, 1724 

%\bibitem[\protect\citeauthoryear{Cortese \& Hughes}{2009}]{Cortese2009} Cortese L., Hughes T.~M., 2009, MNRAS, 400, 1225 


%\bibitem[\protect\citeauthoryear{Cortese et al.}{2011}]{Cortese2011} Cortese L., Catinella B., Boissier S., Boselli A., Heinis S., 2011, MNRAS, 415, 1797 


%\bibitem[\protect\citeauthoryear{DeBoer et al.}{2009}]{DeBoer2009}  DeBoer D.~R., et al., 2009, IEEEP, 97, 1507 


%\bibitem[\protect\citeauthoryear{D{\'e}nes, Kilborn, 
%\& Koribalski}{2014}]{Denes2014} D{\'e}nes H., Kilborn V.~A., Koribalski B.~S., 2014, MNRAS, 444, 667 

\bibitem[\protect\citeauthoryear{D{\'e}nes et al.}{2016}]{Denes2016} D{\'e}nes H., Kilborn V.~A., Koribalski B.~S., Wong O.~I., 2016, MNRAS, 455, 1294 


\bibitem[\protect\citeauthoryear{Dekel et al.}{2009}]{Dekel2009} Dekel A., et al., 2009, Nature, 457, 451 

%\bibitem[\protect\citeauthoryear{Dressler}{1980}]{Dressler1980} Dressler A., 1980, ApJ, 236, 351 


%\bibitem[\protect\citeauthoryear{van Driel $\&$ van Woerden}{1991}]{Driel1991} van Driel W., van Woerden H., 1991, A\&A, 243, 71 

\bibitem[\protect\citeauthoryear{Duc et al.}{2015}]{Duc2015} Duc P.-A., et al., 2015, MNRAS, 446, 120 


%\bibitem[\protect\citeauthoryear{Duffy et al.}{2012}]{Duffy2012}  Duffy A.~R., Meyer M.~J., Staveley-Smith L., Bernyk M., Croton D.~J., 
%Koribalski B.~S., Gerstmann D., Westerlund S., 2012, MNRAS, 426, 3385 

\bibitem[\protect\citeauthoryear{Evslin}{2014}]{Evslin2014} Evslin J., 2014, MNRAS, 440, 1225 

\bibitem[\protect\citeauthoryear{Fabello et al.}{2011}]{Fabello2011} Fabello S., Catinella B., Giovanelli R., Kauffmann G., Haynes M.~P., Heckman T.~M., Schiminovich D., 2011, MNRAS, 411, 993 

%\bibitem[\protect\citeauthoryear{Fernandez et 
%al.}{2015}]{Fernandez2015} Fernandez X., van Gorkom J.~H., Momjian 
%E., Chiles Team, 2015, AAS, 225, $\#$427.03 


%\bibitem[\protect\citeauthoryear{Fraternali et 
%al.}{2002}]{Fraternali2002} Fraternali F., van Moorsel G., Sancisi R., 
%Oosterloo T., 2002, AJ, 123, 3124 

%\bibitem[\protect\citeauthoryear{Fraternali \& Tomassetti}{2012}]{Fraternali2012} Fraternali F., Tomassetti M., 2012, MNRAS, 426, 2166 


\bibitem[\protect\citeauthoryear{Freudling et al.}{2013}]{Freudling2013} Freudling W., Romaniello M., Bramich D.~M., Ballester P., Forchi V., Garc{\'{\i}}a-Dabl{\'o} C.~E., Moehler S., Neeser M.~J., 2013, A\&A, 559, A96 


%\bibitem[\protect\citeauthoryear{Gallazzi et al.}{2008}]{Gallazzi2008} Gallazzi A., Brinchmann J., Charlot S., White S.~D.~M., 2008, MNRAS, 383, 1439 


\bibitem[\protect\citeauthoryear{Ger{\'e}b et al.}{2015}]{Gereb2015} Ger{\'e}b K., Morganti R., Oosterloo T.~A., Hoppmann L., Staveley-Smith L., 2015, A\&A, 580, A43 


\bibitem[\protect\citeauthoryear{Ger{\'e}b et al.}{2016}]{Gereb2016} Ger{\'e}b K., Catinella B., Cortese L., Bekki K., Moran S.~M., Schiminovich D., 2016, MNRAS, 462, 382 

\bibitem[\protect\citeauthoryear{Giovanelli \& Haynes}{1983}]{Giovanelli1983} Giovanelli R., Haynes M.~P., 1983, AJ, 88, 881 


%\bibitem[\protect\citeauthoryear{Giovanelli et %al.}{2005}]{Giovanelli2005} Giovanelli R., et al., 2005, AJ, 130, 2598 

%\bibitem[\protect\citeauthoryear{G{\'o}mez et al.}{2003}]{Gomez2003} G{\'o}mez P.~L., et al., 2003, ApJ, 584, 210 


%\bibitem[van Gorkom $\&$ Schiminovich(1997)]{Gorkom1997} van Gorkom, J., $\&$ Schiminovich, D.\ 1997, The Nature of Elliptical Galaxies; 2nd Stromlo Symposium, 116, 310 



%\bibitem[\protect\citeauthoryear{Hallenbeck et al.}{2014}]{Hallenbeck2014} Hallenbeck G., et al., 2014, AJ, 148, 69 

%\bibitem[\protect\citeauthoryear{Haynes \& Giovanelli}{1984}]{Haynes1984} Haynes M.~P., Giovanelli R., 1984, AJ, 89, 758 


%\bibitem[\protect\citeauthoryear{Haynes et al.}{2011}]{Haynes2011} Haynes M.~P., et al., 2011, AJ, 142, 170 


%\bibitem[\protect\citeauthoryear{Heald et 
%al.}{2011}]{Heald2011} Heald G., et al., 2011, A\&A, 526, A118 


%\bibitem[\protect\citeauthoryear{Hernquist 
%\& Quinn}{1988}]{Hernquist1988} Hernquist L., Quinn P.~J., 1988, ApJ, 331, 682 


%\bibitem[\protect\citeauthoryear{Huang et al.}{2012}]{Huang2012} Huang S., Haynes M.~P., Giovanelli R., Brinchmann J., 2012, ApJ, 756, 113 


\bibitem[\protect\citeauthoryear{Huang et al.}{2014}]{Huang2014} 
Huang S., et al., 2014, ApJ, 793, 40 

\bibitem[\protect\citeauthoryear{van der Hulst \& Sancisi}{1988}]{Hulst1988} van der Hulst T., Sancisi R., 1988, AJ, 95, 1354 



%\bibitem[\protect\citeauthoryear{van der Hulst et al.}{1987}]{Hulst1987} van der Hulst J.~M., Skillman E.~D., Kennicutt R.~C., Bothun G.~D., 1987, A$\&$A, 177, 63 

%\bibitem[\protect\citeauthoryear{van der Hulst $\&$ Sancisi}{1988}]{Hulst1988} van der Hulst T., Sancisi R., 1988, AJ, 95, 1354 

%\bibitem[\protect\citeauthoryear{van der Hulst  \& Sancisi}{2005}]{Hulst2005} van der Hulst J.~M., Sancisi R., 2005, ASPC, 331, 139 


%\bibitem[\protect\citeauthoryear{Ibata et al.}{2001}]{Ibata2001} Ibata R., Irwin M., Lewis G., Ferguson A.~M.~N., Tanvir N., 2001, Natur, 412, 49 

\bibitem[\protect\citeauthoryear{Janowiecki et al.}{2010}]{Janowiecki2010} Janowiecki S., Mihos J.~C., Harding P., Feldmeier J.~J., Rudick C., Morrison H., 2010, ApJ, 715, 972 



\bibitem[\protect\citeauthoryear{Janowiecki et al.}{2015}]{Janowiecki2015} Janowiecki S., et al., 2015, ApJ, 801, 96 


\bibitem[\protect\citeauthoryear{Janowiecki et al.}{2017}]{Janowiecki2017} Janowiecki S., Catinella B., Cortese L., Saintonge A., Brown T., Wang J., 2017, MNRAS,  

\bibitem[\protect\citeauthoryear{Jiang \& Binney}{1999}]{Jiang1999} Jiang I.-G., Binney J., 1999, MNRAS, 303, L7 




%\bibitem[\protect\citeauthoryear{Johnston, Sackett, \& Bullock}{2001}]{Johnston2001} Johnston K.~V., Sackett P.~D., Bullock J.~S., 2001, ApJ, 557, 137 


%\bibitem[\protect\citeauthoryear{Kacprzak \& Churchill}{2011}]{Kacprzak2012} Kacprzak G.~G., Churchill C.~W., 2011, ApJ, 743, L34 

%\bibitem[\protect\citeauthoryear{Karachentsev \& Makarov}{1999}]{Karachentsev1999} Karachentsev I.~D., Makarov D.~I., 1999, IAUS, 186, 109 


\bibitem[\protect\citeauthoryear{Kennicutt}{1989}]{Kennicutt1989} 
Kennicutt R.~C., Jr., 1989, ApJ, 344, 685 

\bibitem[\protect\citeauthoryear{Kennicutt, Kobulnicky, 
\& Pizagno}{1998}]{Kennicutt1998} Kennicutt R.~C., Kobulnicky H.~A., Pizagno J.~L., 1998, AAS, 30, 1354 

\bibitem[\protect\citeauthoryear{Kere{\v s} et 
al.}{2005}]{Keres2005} Kere{\v s} D., Katz N., Weinberg D.~H., 
Dav{\'e} R., 2005, MNRAS, 363, 2 

\bibitem[\protect\citeauthoryear{Kim \& Lee}{2013}]{Kim2013} Kim J.-h., Lee J., 2013, MNRAS, 432, 1701 


%\bibitem[\protect\citeauthoryear{Knapp, Turner, \& Cunniffe}{1985}]{Knapp1985} Knapp G.~R., Turner E.~L., Cunniffe P.~E., 1985, AJ, 90, 454 


\bibitem[\protect\citeauthoryear{Kravtsov}{2013}]{Kravtsov2013} Kravtsov A.~V., 2013, ApJ, 764, L31 


%\bibitem[\protect\citeauthoryear{Larson}{1972}]{Larson1972} Larson 
%R.~B., 1972, Natur, 236, 21 

\bibitem[\protect\citeauthoryear{Lee et al.}{2014}]{Lee2014} Lee C., Chung A., Yun M.~S., Cybulski R., Narayanan G., Erickson N., 2014, MNRAS, 441, 1363 


\bibitem[\protect\citeauthoryear{Lelli, Fraternali, \& Sancisi}{2010}]{Lelli2010} Lelli F., Fraternali F., Sancisi R., 2010, A\&A, 516, A11 

\bibitem[\protect\citeauthoryear{Lemonias et 
al.}{2014}]{Lemonias2014} Lemonias J.~J., Schiminovich D., Catinella 
B., Heckman T.~M., Moran S.~M., 2014, ApJ, 790, 27 

\bibitem[\protect\citeauthoryear{Leroy et al.}{2008}]{Leroy2008} Leroy A.~K., Walter F., Brinks E., Bigiel F., de Blok W.~J.~G., Madore B., Thornley M.~D., 2008, AJ, 136, 2782 

%\bibitem[\protect\citeauthoryear{Lewis et al.}{2002}]{Lewis2002} Lewis I., et al., 2002, MNRAS, 334, 673 

\bibitem[\protect\citeauthoryear{Lutz et al.}{2017}]{Lutz2017} Lutz K.~A., et al., 2017, MNRAS,  


%\bibitem[\protect\citeauthoryear{Malin \& Hadley}{1997}]{Malin1997} Malin D., Hadley B., 1997, PASA, 14, 52 

\bibitem[\protect\citeauthoryear{Mapelli, Rampazzo, \& Marino}{2015}]{Mapelli2015} Mapelli M., Rampazzo R., Marino A., 2015, A\&A, 575, A16 


\bibitem[\protect\citeauthoryear{Martig et al.}{2009}]{Martig2009} Martig M., Bournaud F., Teyssier R., Dekel A., 2009, ApJ, 707, 250 


\bibitem[\protect\citeauthoryear{Martin et al.}{2005}]{Martin2005} Martin D.~C., et al., 2005, ApJ, 619, L1 

\bibitem[\protect\citeauthoryear{Mart{\'{\i}}nez-Delgado et al.}{2010}]{Martinez2010} Mart{\'{\i}}nez-Delgado D., et al., 2010, AJ, 140, 962 


%\bibitem[\protect\citeauthoryear{Martin et al.}{2012}]{Martin2012} Martin C.~L., Shapley A.~E., Coil A.~L., Kornei K.~A., Bundy K., Weiner B.~J., Noeske K.~G., Schiminovich D., 2012, ApJ, 760, 127 

%\bibitem[\protect\citeauthoryear{McConnachie et al.}{2003}]{McConnachie2003} McConnachie A.~W., Irwin M.~J., Ibata R.~A., Ferguson A.~M.~N., Lewis G.~F., Tanvir N., 2003, MNRAS, 343, 1335 


\bibitem[\protect\citeauthoryear{McMullin et al.}{2007}]{McMullin2007} McMullin J.~P., Waters B., Schiebel D., Young W., Golap K., 2007, ASPC, 376, 127 


%\bibitem[\protect\citeauthoryear{Meyer et al.}{2004}]{Meyer2004} Meyer M.~J., et al., 2004, MNRAS, 350, 1195 


%\bibitem[\protect\citeauthoryear{Morganti et al.}{1997}]{Morganti1997} Morganti R., Sadler E.~M., Oosterloo T., Pizzella A., Bertola F., 1997, AJ, 113, 937 


%\bibitem[\protect\citeauthoryear{Morganti et al.}{2006}]{Morganti2006} Morganti R., et al., 2006, MNRAS, 371, 157 

\bibitem[\protect\citeauthoryear{Mo, Mao, \& White}{1998}]{Mo1998} Mo H.~J., Mao S., White S.~D.~M., 1998, MNRAS, 295, 319 

\bibitem[\protect\citeauthoryear{Moran et al.}{2010}]{Moran2010} Moran S.~M., et al., 2010, ApJ, 720, 1126 


\bibitem[\protect\citeauthoryear{Morganti}{2007}]{Morganti2007} Morganti R., 2007, mcct.conf, 12 


% \bibitem[\protect\citeauthoryear{Oosterloo, Fraternali, \& Sancisi}{2007}]{Oosterloo2007} Oosterloo T., Fraternali F., Sancisi R., 2007, AJ, 134, 1019 

%\bibitem[\protect\citeauthoryear{Oosterloo et al.}{2010a}]{Oosterloo2010} Oosterloo T., et al., 2010a, MNRAS, 409, 500 
\bibitem[\protect\citeauthoryear{Oosterloo et al.}{2010}]{Oosterloo2010} Oosterloo T., et al., 2010, MNRAS, 409, 500 



%\bibitem[\protect\citeauthoryear{Oosterloo, Verheijen, \& van Cappellen}{2010b}]{Oosterloo2010b} Oosterloo T., Verheijen M., van Cappellen W., 2010b, iska.meet, 43 

\bibitem[\protect\citeauthoryear{Naab \& Burkert}{2001}]{Naab2001} Naab T., Burkert A., 2001, ApJ, 555, L91 

\bibitem[\protect\citeauthoryear{Nelson et al.}{2015}]{Nelson2015} Nelson D., et al., 2015, A\&C, 13, 12 


\bibitem[\protect\citeauthoryear{Pickering et al.}{1997}]{Pickering1997} Pickering T.~E., Impey C.~D., van Gorkom J.~H., Bothun G.~D., 1997, AJ, 114, 1858 


\bibitem[\protect\citeauthoryear{Obreschkow et al.}{2016}]{Obreschkow2016} Obreschkow D., Glazebrook K., Kilborn V., Lutz K., 2016, ApJ, 824, L26 



%\bibitem[\protect\citeauthoryear{Ostriker \& Binney}{1989}]{Ostriker1989} Ostriker E.~C., Binney J.~J., 1989, MNRAS, 237, 785 


%\bibitem[\protect\citeauthoryear{Querejeta et al.}{2015}]{Querejeta2015} Querejeta M., et al., 2015, A$\&$A, 579, L2 

%\bibitem[\protect\citeauthoryear{Roberts \& Haynes}{1994}]{Roberts1994} Roberts M.~S., Haynes M.~P., 1994, ARA\&A, 32, 115 


%\bibitem[\protect\citeauthoryear{Rots et al.}{1990}]{Rots1990} Rots A.~H., Bosma A., van der Hulst J.~M., Athanassoula E., Crane P.~C., 1990, AJ, 100, 387 


%\bibitem[\protect\citeauthoryear{Sadler, Oosterloo, \& Morganti}{2002}]{Sadler2002} Sadler E.~M., Oosterloo T., Morganti R., 2002, ASPC, 273, 215 

\bibitem[\protect\citeauthoryear{Robertson et al.}{2006}]{Robertson2006} Robertson B., Cox T.~J., Hernquist L., Franx M., Hopkins P.~F., Martini P., Springel V., 2006, ApJ, 641, 21 


\bibitem[\protect\citeauthoryear{Saintonge et al.}{2011}]{Saintonge2011} Saintonge A., et al., 2011, MNRAS, 415, 32 


%\bibitem[\protect\citeauthoryear{Salpeter}{1955}]{Salpeter1955} Salpeter E.~E., 1955, ApJ, 121, 161 


\bibitem[\protect\citeauthoryear{Sancisi et 
al.}{2008}]{Sancisi2008} Sancisi R., Fraternali F., Oosterloo T., van der Hulst T., 2008, A\&ARv, 15, 189 

\bibitem[\protect\citeauthoryear{Schaye et al.}{2015}]{Schaye2015} Schaye J., et al., 2015, MNRAS, 446, 521 

\bibitem[\protect\citeauthoryear{Schawinski et al.}{2014}]{Schawinski2014} Schawinski K., et al., 2014, MNRAS, 440, 889 

\bibitem[\protect\citeauthoryear{Schiminovich et al.}{2010}]{Schiminovich2010} Schiminovich D., et al., 2010, MNRAS, 408, 919 

\bibitem[\protect\citeauthoryear{Schmidt}{1959}]{Schmidt1959} 
Schmidt M., 1959, ApJ, 129, 243 


\bibitem[\protect\citeauthoryear{Seibert et al.}{2012}]{Seibert2012} Seibert M., et al., 2012, AAS, 219, 340.01 


\bibitem[\protect\citeauthoryear{Serra et al.}{2006}]{Serra2006} Serra P., Trager S.~C., van der Hulst J.~M., Oosterloo T.~A., Morganti R., 2006, A\&A, 453, 493 

\bibitem[\protect\citeauthoryear{Serra et al.}{2012}]{Serra2012} Serra P., et al., 2012, MNRAS, 422, 1835 

%\bibitem[\protect\citeauthoryear{Simkin, Su, \& Schwarz}{1980}]{Simkin1980} Simkin S.~M., Su H.~J., Schwarz M.~P., 1980, ApJ, 237, 404 


\bibitem[\protect\citeauthoryear{Simkin et al.}{1987}]{Simkin1987} Simkin S.~M., van Gorkom J., Hibbard J., Su H.-J., 1987, Sci, 235, 1367 


\bibitem[\protect\citeauthoryear{Solanes et al.}{2001}]{Solanes2001} Solanes J.~M., Manrique A., Garc{\'{\i}}a-G{\'o}mez C., Gonz{\'a}lez-Casado G., Giovanelli R., Haynes M.~P., 2001, ApJ, 548, 97 


\bibitem[\protect\citeauthoryear{Spavone et al.}{2010}]{Spavone2010} Spavone M., Iodice E., Arnaboldi M., Gerhard O., Saglia R., Longo G., 2010, ApJ, 714, 1081 

\bibitem[\protect\citeauthoryear{Springel \& Hernquist}{2005}]{Springel2005} Springel V., Hernquist L., 2005, ApJ, 622, L9 


%\bibitem[\protect\citeauthoryear{Thakar et al.}{1997}]{Thakar1997} Thakar A.~R., Ryden B.~S., Jore K.~P., Broeils A.~H., 1997, ApJ, 479, 702 


%\bibitem[\protect\citeauthoryear{Toomre $\&$ Toomre}{1972}]{Toomre1972} Toomre A., Toomre J., 1972, ApJ, 178, 623 


%\bibitem[\protect\citeauthoryear{Twarog}{1980}]{Twarog1980} Twarog B.~A., 1980, ApJ, 242, 242 


%\bibitem[\protect\citeauthoryear{Veron-Cetty et al.}{1995}]{Veron1995} Veron-Cetty M.-P., Woltjer L., Ekers R.~D., Staveley-Smith L., 1995, A$\&$A, 297, L79 

%\bibitem[\protect\citeauthoryear{Wang et al.}{2010}]{Wang2010} Wang J., Overzier R., Kauffmann G., von der Linden A., Kong X., 2010, MNRAS, 401, 433 


%\bibitem[\protect\citeauthoryear{Wang et al.}{2013}]{Wang2013} Wang J., et al., 2013, MNRAS, 433, 270

\bibitem[\protect\citeauthoryear{Wang et al.}{2015}]{Wang2015} Wang J., et al., 2015, MNRAS, 453, 2399 
 

%\bibitem[\protect\citeauthoryear{Wardle \& Knapp}{1985}]{Wardle1985} Wardle M.~J., Knapp G.~R., 1985, BAAS, 17, 611 

\bibitem[\protect\citeauthoryear{Wyder et al.}{2007}]{Wyder2007} Wyder T.~K., et al., 2007, ApJS, 173, 293 


\bibitem[\protect\citeauthoryear{van Woerden, van Driel, \& Schwarz}{1983}]{vanWoerden1983} van Woerden H., van Driel W., Schwarz U.~J., 1983, IAUS, 100, 99 

\bibitem[\protect\citeauthoryear{York et al.}{2000}]{York} York D.~G., et al., 2000, AJ, 120, 1579 

%\bibitem[\protect\citeauthoryear{Yun, Ho, \& Lo}{1994}]{Yun1994} Yun M.~S., Ho P.~T.~P., Lo K.~Y., 1994, Natur, 372, 530 


\bibitem[\protect\citeauthoryear{Zibetti, Charlot, $\&$ Rix}{2009}]{Zibetti2009} Zibetti S., Charlot S., Rix H.-W., 2009, MNRAS, 400, 1181 

%\bibitem[\protect\citeauthoryear{Zwaan et al.}{2005}]{Zwaan2005} Zwaan M.~A., Meyer M.~J., Staveley-Smith L., Webster R.~L., 2005, MNRAS, 359, L30 



\end{thebibliography}







==> Tex_files/Environment.tex <==
\subsection{Environment}\label{Sec:env}

It has been known for several decades that high density environments, such as clusters, play a very important role when it comes to gas removal processes \citep{Giovanelli1983, Solanes2001, Catinella2013, Denes2016}. Low-density environments, on the other hand, provide favourable conditions for galaxies to accumulate gas \citep{Wang2015, Janowiecki2017}. In Paper I we show that GASS 3505 lives in a low density environment populated by gas-rich galaxies, the perfect neighbourhood for building and maintaining a large gas reservoir. 
Now we examine the observed volume around the other four \HI-excess galaxies both in \HI\ and in the SDSS spectroscopic catalog. Our sample is selected against \HI\ confusion within the ALFALFA beam, therefore we avoid the densest environments by selection.

We find two galaxies in the vicinity of GASS 20339 with available SDSS spectroscopy, however the galaxies are not detected in \HI\ at the $3\sigma$ upper limit of log$(M_{\rm HI}) < 9.6 $ \msun\ (assuming a line width of 200 \kms). These galaxies are marked as red boxes in Fig. \ref{fig:G20339_env}. The \HI\ non-detections are likely due to the fact that these galaxies are located in high-noise regions of the cube, far away from the phase centre where the sensitivity declines due to the effect of the primary beam.

In the environment of J1126 we find two \HI\ detections with faint optical counterparts in SDSS, see Fig. \ref{fig:J1126_env}. Interestingly, these dwarf galaxies do not have optical spectroscopy, similarly to the cases found in the neighbourhood of GASS 3505. The \HI\ detection of the dwarf in the north is discussed in Sec. \ref{Sec:HIprop}. The second galaxy has an \HI\ mass of log$(M_{\rm HI}) = 9.1$ \msun.  

We also find an \HI\ detection nearby J1558 with SDSS spectroscopy, and we measure its \HI\ mass to be log$(M_{\rm HI}) = 9.7$ \msun. The environment of J1558 is shown in Fig. \ref{fig:J1558_env}.

J1605 does not have any SDSS or \HI-detected neighbours, therefore we do not show a map of this galaxy in the Appendix. 

These examples support the results found for GASS 3505, that \HI-excess galaxies are typically found in low-density environments. Even though we are still limited by number statistics, it appears that optically faint dwarf galaxies are often found in the vicinity of such \HI\ beasts. However, control samples are needed to address whether \HI-excess galaxies are exceptional in this sense, or optically faint companions are typical for all (massive) galaxies. The \HI\ masses detected in dwarf galaxies are too low to push galaxies into the \HI-excess regime once accreted, however these are clearly contributing in some cases. 


   
%\begin{table}
%  \caption{Properties of galaxies in the environment of the \HI-excess sample - {\bf to be completed}. Col.1 SDSS identification number; Col.2 redshift; Col.3 projected distance from the central galaxy; Col.4 stellar mass; Col.5 \HI\ mass}\label{table:summary}
  
%   \begin{center}
%     \begin{tabular}{c c c c c} 		
    %&  & References\\ 	
%\hline									     
%SDSS ID  & z  & $d_{\rm proj}$ & log($M_{\star}$) & log($M_{\rm \HI}$)  \\ 
%         &    &  kpc           &   [\msun]        &  [\msun]            \\
%\hline	
% &  &  &  &   \\ 
%     &  &  &  &  \\
%    &  &  &  &  \\
%    &  &  &  &   \\

%\end{tabular}


    %\begin{tablenotes}
   %  {\bf References.} (1) Catinella et al. (2010); (2) Saintonge et al. (2011a)
    % \item[$\dagger$]  The stellar mass is from SDSS.
    	%\end{tablenotes
%\end{center}
%\end{table}



%- Environment: SDSS images overlayed with detections and non-detections. GASS 20339 has X detected and Y non-detected...The same for the others... Any of these gravitationally bound?
%All isolated centrals in Yang., although we detect a few dwarf galaxies without SDSS spectra, for example near GASS 3505 and J1126. These galaxies live in a low-density environement of gas-rich galaxies, perfect for building and mainting the \HI-excess gas reservoirs.




==> Tex_files/HIproperties.tex <==

\section{The HI data}\label{Sec:HIprop}


==> Tex_files/KSrelation.tex <==

\section{The low end of the KS relation}\label{Sec:HIprop}


==> Tex_files/UVproperties.tex <==


